LEAPER: Fast and Accurate FPGA-based System Performance Prediction via Transfer Learning

Machine learning has recently gained traction as a way to overcome the slow accelerator generation and implementation process on an FPGA. It can be used to build performance and resource usage models that enable fast early-stage design space exploration. First, training requires large amounts of data (features extracted from design synthesis and implementation tools), which is cost-inefficient because of the time-consuming accelerator design and implementation process. Second, a model trained for a specific environment cannot predict performance or resource usage for a new, unknown environment. In a cloud system, renting a platform for data collection to build an ML model can significantly increase the total-cost-ownership (TCO) of a system. Third, ML-based models trained using a limited number of samples are prone to overfitting. To overcome these limitations, we propose LEAPER, a transfer learning-based approach for prediction of performance and resource usage in FPGA-based systems. The key idea of LEAPER is to transfer an ML-based performance and resource usage model trained for a low-end edge environment to a new, high-end cloud environment to provide fast and accurate predictions for accelerator implementation. Experimental results show that LEAPER (1) provides, on average across six workloads and five FPGAs, 85% accuracy when we use our transferred model for prediction in a cloud environment with 5-shot learning and (2) reduces design-space exploration time for accelerator implementation on an FPGA by 10x, from days to only a few hours.

==> LEAPER_ICCD'22_Camera_ready_FINAL/abstract_submit.tex <==
Machine learning has recently gained traction as a way to overcome the slow accelerator generation and implementation process on an FPGA. It can be used to build performance and resource usage models that enable fast early-stage design space exploration. First, training requires large amounts of data (features extracted from design synthesis and implementation tools), which is cost-inefficient because of the time-consuming accelerator design and implementation process.  Second, a model trained for a specific environment cannot predict performance or resource usage for a new, unknown environment. In a cloud system, renting a platform for data collection to build an ML model can significantly increase the total-cost-ownership (TCO) of a system. Third, ML-based models trained using a limited number of samples are prone to overfitting. To overcome these limitations, we propose LEAPER, a transfer learning-based approach for prediction of performance and resource usage in FPGA-based systems. The key idea of LEAPER is to transfer an ML-based performance and resource usage model trained for a low-end edge environment to a new, high-end cloud environment to provide fast and accurate predictions for accelerator implementation. Experimental results show that LEAPER (1) provides, on average across six workloads and five FPGAs, 85% accuracy when we use our transferred model for prediction in a cloud environment with 5-shot learning and (2) reduces design-space exploration time for accelerator implementation on an FPGA by 10x, from days to only a few hours.

==> LEAPER_ICCD'22_Camera_ready_FINAL/algorithms/transfer_algorithm.tex <==
% \begin{figure}[h]
%   \centering
% \begin{minipage}{\linewidth}
% \centering
% {%\fontsize{7.8}{10}\selectfont
\begin{algorithm}[h]
 \caption{\namePaper's~transfer learning \gs{algorithm.}}
%  \caption{\namePaper's~adaptive transfer learning}
\setstretch{0.55}
\small
 \label{algo:transfer}
\SetAlgoLined\DontPrintSemicolon
 \SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
  \KwIn{(1) Base model ($f_s$) trained \ommm{on} the edge environment,\\  \hskip3em (2) Sub-sampled {\emph{few-shot learning} dataset $c_{tl}\subset c_{doe}$\\ \hskip3em from the base and the target environment}}   %$c_{tl}\subset c_{lhs}$
  \KwOut{Target {cloud} model ${f}_t:\mathcal{X}_t \to \mathcal{Y}_t$}
\textbf{Initialize:} Maximum number of iterations M\label{algo:tl_initial}\;
\While{$M\not=0$}{\label{algo:tl_initial_loop}
    Normalize the feature vector\label{algo:tl_data}\;
    Train ensemble transfer learners (TL) with $c_{tl}$\label{algo:tl_train}\;
   Find the candidate TL:\;\hskip1em  $\hat{h}_t:\mathcal{X}_{tl} \to \mathcal{Y}_{tl}$ that minimizes the error over the $c_{doe}-c_{tl}$\; \label{algo:line:findTL}
    Compute the mean relative error\label{algo:tl_mre}: \\
   \hskip1em $\epsilon_{mre}=\frac{1}{c_{doe}-c_{tl}} \displaystyle\sum_{i=1}^{c_{doe}-c_{tl}} \frac{|y_{t}^{acc} -y_{t}^{pred}|}{y_{t}^{acc}}$
   
    Use identified $\hat{h}_t$ to transform predictions of $f_s$:\label{algo:tl_transform}\\
   \hskip1em${f}_t$=$\hat{h}_t(f_s)$  \label{algo:tl_transfer_predict} \hskip7em where $f_s: \mathcal{X}_s \to \mathcal{Y}_s$\\
   $M \leftarrow M - 1$
}
\textbf{return}  ${f}_t$
\end{algorithm}
% }
% \end{minipage}
% \end{figure}

==> LEAPER_ICCD'22_Camera_ready_FINAL/commands.tex <==
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0pt,fill=black, text=white] (char) {#1};}}
\newcommand*\circledWhite[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0pt,fill=white, text=black] (char) {#1};}}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

  
\definecolor{dred}{rgb}{0.75, 0.00, 0.00}
\definecolor{dgreen}{rgb}{0.00, 0.5, 0.00}
\definecolor{ddgreen}{rgb}{0.00, 0.50, 0.00}
\definecolor{dpink}{rgb}{0.75, 0.0, 0.75}
\definecolor{dblack}{rgb}{0.00, 0.00, 0.00}
\definecolor{dblue}{rgb}{0.00, 0.00, 0.75}
\definecolor{gyell}{rgb}{0.5, 0.5, 0.0}
\definecolor{dbleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{darkgoldenrod}{rgb}{0.72, 0.53, 0.04}
\definecolor{magenta}{rgb}{160,0,255}
\newcommand{\jgl}[1]{[{\color{dgreen}JGL: #1}]}
\newcommand{\juan}[1]{{\color{black}#1}}
\newcommand{\juang}[1]{{\color{black}#1}}
\newcommand{\gagan}[1]{{\color{black}#1}}
\newcommand{\gs}[1]{{\color{black}#1}}
\newcommand{\gss}[1]{{\color{black}#1}}
\newcommand{\om}[1]{{\color{black}#1}}
\newcommand{\omm}[1]{{\color{black}#1}}
\newcommand{\ommm}[1]{{\color{black}#1}}
\newcommand{\omu}[1]{{\color{black}#1}}
\newcommand{\gaganT}[1]{{\color{black}#1}}
\newcommand{\did}[1]{{\color{black}#1}}
% ---------------------------------------------------    
%% Version header
%  \usepackage[font=small,labelfont=bf]{caption}
% \usepackage{fancyhdr}
% \usepackage{datetime}
% %% Version header 
% \newcommand{\versionnum}[0]{2.7}
% \fancypagestyle{plain}{
%   \fancyhf{}% Clear header/footer
%   \fancyhead[C]{\textcolor{dblue}{\emph{Version \versionnum~---~\today, \ampmtime}}}
%   \fancyfoot[C]{\thepage}% Right footer
% }
% \pagestyle{plain}% Set page style to plain.
% %---------------------------------------------------  

\renewcommand{\baselinestretch}{1}
\newcommand{\head}[1]{{\noindent\textbf{#1.}\xspace}} % for
\newcommand{\namePaper}{LEAPER\xspace} %TITLE FOR THE PAPER
\newcommand{\etal}{\textit{et al.}}
\setstretch{0.85}

==> LEAPER_ICCD'22_Camera_ready_FINAL/images/LHS.tex <==
\begin{SCfigure}[][h]
\vspace{0.8cm}
\centering
    \resizebox{0.3\textwidth}{!}{
    
    
    \begin{tikzpicture}
    %[rotate=90,transform shape]

\draw[step=0.25cm,gray,very thin] (0,0) grid (2,2);

\draw[thick,->] (0,0) -- (2.4,0);
\draw[thick,->] (0,0) -- (0,2.2);
%  \node at (0,0) [circle,fill=black] {};
%  \filldraw [gray] (0,0.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (2,2) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.25,1.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.75,0) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1,1.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.75,0.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.5,0.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.25,1.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0,1) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.5,0.5) circle (2pt);


 
 
\node at (0,2.4)[ rotate=0] {\small \textit{x1}};
\node at (2.6,0)[ rotate=0] {\small \textit{x2}};
\end{tikzpicture}
}
\vspace{-1cm}
\caption{LHS with 2 parameters where the input space is divided into equal intervals and 9 non-overlapping sample points are chosen.
\label{fig:LEAPER_SIGMETRICS/LHS}}
\end{SCfigure}


==> LEAPER_ICCD'22_Camera_ready_FINAL/packages.tex <==
% \usepackage[a4paper,top=25mm,bottom=20mm, width=170mm,bindingoffset=6mm]{geometry}  
%\usepackage[english]{babel}
% \usepackage[utf8]{inputenc}
%\usepackage{fancyhdr}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{listings}
\usepackage{caption}
\usepackage{balance}
\usepackage{threeparttable,booktabs}
\usepackage[algoruled,resetcount,linesnumbered ]{algorithm2e}

% \captionsetup[equa]{font={bf}}
% \captionsetup[lstlisting]{font={bf}}
% \captionsetup[figure]{labelfont={bf}}
% \captionsetup[figure]{font={small}}
% \captionsetup[table]{labelfont={bf}}
% \captionsetup[table]{font={small,stretch=0.9}}
\setlength{\footnotesep}{0.01\footnotesep}
\newcommand{\note}[1]{\footnote{\setstretch{0.22}#1}}
%  \captionsetup[figure]{font={bf}}
% \captionsetup[table]{font={bf}}
\usepackage{float}
\usepackage{amsmath}
\usepackage{tikz}
\usetikzlibrary{automata,arrows,topaths, shapes}
\usepackage{siunitx}
% \usepackage{subfigure}
% \usepackage[subfigure]{tocloft}
% \usepackage[toc,page]{appendix}
\usepackage{hyperref}
\usepackage{subcaption}
\usepackage{parcolumns}
\usepackage{soul}
\usepackage{eso-pic,lipsum}
\hypersetup{
    colorlinks=false,
    pdfborder={0 0 0},
}

\usepackage{ragged2e}   % to undo \centering
\usepackage{glossaries}
% define list of equations
\usepackage{booktabs}

\usepackage{multirow}
%  \newcommand{\xAlCapSty}[1]{\small\textbf{#1}}
%  \SetAlCapSty{xAlCapSty}
% command to box, label, reference, and 
% include noteworthy equation in list of equations


%%%%%%%%%%%%%%%%%% END COLORS DEFINITION %%%%%%%%%%%%%%%%%% 


%%%%%%%%%%%%%%%%%% COMMENTS MACRO  %%%%%%%%%%%%%%%%%% 
%\usepackage{xargs}
%\usepackage[textsize=footnotesize]{todonotes}
%\newcommandx{\chelini}[2][1=]{#1\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{\textbf{Chelini: } #2}}
%\paperwidth=\dimexpr \paperwidth + 12cm\relax    \oddsidemargin=\dimexpr\oddsidemargin + 6cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 6cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 6cm\relax
%\setlength{\marginparwidth}{7cm}
%%%%%%%%%%%%%%%%%% END COMMENTS MACRO  %%%%%%%%%%%%%%%%%% 


	% MINESH: SQUEEZE in a way that doesn't mandate vspace
	\makeatletter
	\g@addto@macro{\normalsize}{%
	  \setlength{\abovedisplayskip}{2pt plus 1pt minus 1pt}
	  \setlength{\belowdisplayskip}{2pt plus 1pt minus 1pt}
	  \setlength{\abovedisplayshortskip}{0pt}
	  \setlength{\belowdisplayshortskip}{0pt}
	  \setlength{\intextsep}{2pt plus 1pt minus 1pt}
	  \setlength{\textfloatsep}{4pt plus 1pt minus 1pt}
	  \setlength{\skip\footins}{5pt plus 1pt minus 1pt}}
	  \setlength{\abovecaptionskip}{3pt plus 1pt minus 1pt}
	\makeatother
	\usepackage{titlesec}

\makeatletter
\def\endthebibliography{%
  \def\@noitemerr{\@latex@warning{Empty `thebibliography' environment}}%
  \endlist
}
\usepackage{setspace}

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{sidecap}

\usepackage{tikz}

\usepackage{enumitem}

% Version header 
 \usepackage{fancyhdr}
%  \usepackage[us,12hr]{datetime}



\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
    



\usepackage[hang,flushmargin]{footmisc}

==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/abstract.tex <==
\begin{abstract}
Machine learning %-based models have 
 \omm{has} recently gained traction as a way to overcome the slow \om{accelerator generation and implementation process on an FPGA}. %downstream implementation process of FPGAs 
\juang{It can be used to build} \om{performance and resource \ommm{usage}} models that \om{enable fast early-stage design space exploration}. %provide fast and accurate performance predictions. 
However, these models suffer from \omm{three} main limitations. %: (1) 
\juang{First,} training requires large amounts of data (features extracted from design synthesis and implementation tools), which is cost-inefficient because of the time-consuming \om{accelerator} design \om{and implementation process}. %; (2) 
\juang{Second,} a model trained for a specific environment cannot predict \om{performance} %(resource utilization)} 
\juang{or resource \ommm{usage}} for a new, unknown environment. In a cloud system, 
%where getting access to platforms is typically costly, 
\om{renting a platform for} data collection \om{to build an} ML model can significantly increase the total-cost-ownership (TCO) of a system. \omm{Third, ML-based models trained using a limited number of samples are prone to overfitting.} To overcome these limitations, we propose \namePaper, a \textit{transfer learning}-based approach for \juang{prediction of performance and resource \ommm{usage} in} FPGA-based systems. %that 
\juang{The key idea of \namePaper is to transfer} %adapts 
an ML-based performance and resource \ommm{usage} model \om{trained for a low-end edge environment} to a new, high-end cloud environment to provide fast and accurate predictions \om{for %an 
accelerator implementation}. 
Experimental results show that \om{\namePaper} %delivers
\juang{(1) provides}, on average \juang{across six workloads and five FPGAs}, 85\% accuracy {when we use our transferred model for prediction in a cloud environment} with \textit{5-shot learning} and \juang{(2)} reduces {design-space exploration} time \om{for %an 
accelerator implementation on an FPGA} by 10$\times$, from days to {only} a few hours. 









% Machine learning-based models have recently gained traction to overcome the notoriously slow downstream implementation process of FPGAs. However, an ML-based model trained for a specific environment cannot predict for a new environment. Moreover, traditional ML approaches require large amounts of training data, which is cost-inefficient owing to the time-consuming FPGA design cycle. We propose \namePaper, a transfer learning-based approach for heterogeneous systems augmented with intelligent statistical techniques. It overcomes the inefficiency of ML-based approaches by adapting an existing ML-based model for a new environment by retraining with only a few samples.
% Experimental results show that our approach
% delivers 80-90\% accuracy on average with few-shots, and it expedites DSE by 14$\times$, reducing from several days to a few hours. 

% Once transferred, the model can quickly provide accurate results across different environments. Experimental results show that our approach
% delivers 80\% accuracy on average with few-shots, and it expedites DSE by 14$\times$. 
% \gaganCheck{*Need to reduce the abstract, RIGHT now 123 words, shouldn't be more than 100 words}

% Modern CPU-FPGA based heterogeneous systems provide developers with increasingly large
% design options \jgl{Why is that?}. However, FPGA development has low productivity and tool run-times are cost-prohibitive for effective
% design space exploration \juan{DSE}, preventing designers from making approapriate decisions without expert guidance. 
% Several machine learning based models have been proposed to overcome this issue \jgl{What do this models provide?}. 
% However, these traditional approaches are data hungry that are trained for specific platform and hence these models become useless when deployed to new hardware targets.  Naturally, this does not scale when relying on real measurements in the changing environments, i.e., they are highly cost-inefficient. 
% \jgl{State the problems clearly: 1) An ML-based model trained for a specific platform is incapable of estimating performance for a new platform; 2) Training for a new platform requires a large amount of training data.}

% To this end \jgl{What is the end? You are not really stating your goal.} we propose RECOIL, a transfer-learning-based approach for heterogeneous systems that can overcome this inefficiency of traditional ML-based approaches by %adapting the old ML model to a new task by using a few samples only. 
% \juan{adapting an existing ML-based performance estimation model for a new system by retraining with only a few samples.} 
% Once transferred, the model can %be used to 
% quickly provide \juan{accurate} performance results across different configurations. 
% In order to minimize the data collection overhead for DSE, this paper proposes an efficient DSE method which combines Latin hypercube sampling and an adaptive ensemble transfer learning technique. Our experiments show we are able to develop cheaper, faster and accurate performance models for performance prediction in changing environments. Experimental results show that our approach
% delivers 80 to 90\% accuracy with few-shots (5 samples) and is able to explore 14$\times$ faster the entire design space across various platforms.

\end{abstract}

==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/conclusion.tex <==
\section{Conclusion}
% \vspace{-0.1cm}
% Modern CPU-FPGA %based 
% heterogeneous systems provide developers with extensive design options to optimize an application. However, FPGA development has low productivity, and tool run-times are cost-prohibitive for practical design space exploration (DSE). %Thus, preventing designers from making 
% {This makes difficult for designers to make} appropriate decisions without expert guidance. 

%To this end, 
% {To avoid these shortcomings,} 
We introduce \namePaper, {the first} \textit{transfer learning}-based approach \ommm{for prediction of performance and resource usage in FPGA-based systems. % \namePaper combines statistical techniques and transfer learning to minimize the ML training data collection overhead.  
\namePaper overcomes the inefficiency of traditional ML-based methods by leveraging an ML-based performance and resource \ommm{usage} model trained for a low-end \om{edge environment} to predict \omu{the} performance and resource \ommm{usage} of an accelerator implementation for a new, high-end cloud environment.}

% Traditional ML-based approaches have the following two shortcomings: 1) an ML-based model trained for a specific environment (application or hardware) is incapable of estimating {the} performance for a new {unknown} environment, and 2) training for a new environment requires a large amount of training data.
 
 Our experiments show that \ommm{\namePaper is} cheaper (with \textit{5-shot}), faster (up to $10\times$), and highly accurate (on average 85\%)  \ommm{at predicting} performance and resource \ommm{usage} in a new, {unknown} target {cloud} environment \ommm{than building models from scratch}. 
%  LHS reduces training samples from 500+ to 50, while  \textit{5-shot} learning further reduces this space to 5, so we achieve $100\times$ effective speedup compared to a conventional brute-force approach. %In the future, we would extend 
 We believe that \namePaper~\ommm{can} open up new avenues for research on FPGA-based systems from edge to cloud computing, and hopefully, \ommm{it will} inspire the development of new modeling techniques \ommm{for FPGAs}. %other alternatives to traditional ML-based models.

% Another exciting direction would be to evaluate the applicability of transfer learning to a virtualized environment.

% Moreover, we show that with limited time budget, our methods are more suitbale than state-of-the-art supervised learning methods. We are able to generalize from a few examples.

% FPGA ML

% Predicting parallel application performance via machine learning approaches





% "The analytical
% models require a-priori knowledge of performance indicators as a precursor to model construction.
% Predictive models, in contrast, do not require this information, although do require the usage of a
% golden reference values during training"

% One of the key advantages of using a model to learn patterns
% that generalize (as opposed to lookup tables) is that the
% model can then be introspected in order to gain insights into
% the data


% As k gets larger, the difference in size between the training set and the resampling subsets gets smaller. As this difference decreases, the bias of the technique becomes smaller


% the behavior of one program can differ wildly from that of another.2. (In fact, the behavior of a single program can behave wildly different from one input
% to another. For example, consider how the behavior of gcc differs when compiling, say,
% matrix multiplication as opposed to an OS)



% We extract information from the source
% model that guides the sampling in the target environment, to gather
% fewer but more informative samples, and therefore, to gain a better
% understanding of the system performance with less cost.



==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/discussion.tex <==
\section{Discussion and Limitations}
 \label{section:limit}


\head{\namePaper's~generality}
\namePaper is a framework for building and transferring models from a small edge environment to any new, unknown FPGA-based environment. We demonstrate our approach using the cloud system as our target environment because cloud systems often use expensive, high-end FPGAs, e.g., Amazon AWS~F1 cloud~\cite{aws}, Alibaba Elastic cloud~\cite{alibaba}, etc. We can, thus, achieve tangible gains in terms of cost, efficiency, and performance. However, \namePaper can be used to transfer models to any high-end FPGA system.


\noindent\textbf{Effect of FPGA resource saturation.}
% Our primary focus was to use a low-cost FPGA-board (available offline) for building a model using traditional ML technique and then leverage transfer-learning to reuse the same model for prediction of high-end server-grade FPGAs (e.g., in the cloud, where data collection could be expensive or even error-prone). Our approach dramatically reduces the number of costly trials on the high-end FPGA. We limit ourselves to designs that fit on the small FPGA capacity because the major contribution of this approach lies in the ability to transfer learning from low-end edge FPGA to high-end cloud FPGAs. 
An FPGA gives us the flexibility to map \ommm{a given} operation to different \ommm{potential} resources. For example, we can map a multiplication operation  to either a CLB or a DSP slice. \ommm{We can decide the mapping based on the operand width, i.e., if the operand width is smaller than DSP slice width, the operation is mapped to a CLB otherwise to a DSP unit.} %An ML-based model can be trained to learn such relations. 
\ommm{Currently, we do not consider mapping the same operation to different resources.}


% \noindent\textbf{FPGA resource constrained environments.}
% We evaluate bare-metal systems without a middleware layer. In a multi-tenant environment~\cite{pourhabibi2020optimus} or during partial reconfiguration~\cite{beckhoff2012go} we are often constrained by limited resources~\cite{ting2020dynamic}. In such scenarios, the resource management is more efficient to be controlled by a middleware layer~\cite{vaishnav2020fos}. In future, we aim to extend our work to such scenarios as well.

\head{Transfer a model to a new platform and application simultaneously}
In supervised learning, transferring both to a new platform and application at the same time would lead to sub-optimal results (as observed in~\cite{xapp}). This sub-optimal performance is because in such a scenario we would perform two \ommm{types} of transfer \ommm{at the same time to (1)} unknown hardware and (2) unknown application. % an ML model needs to have some notion of the target environment. 
We explicitly exclude this scenario in the current work.

==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/introduction.tex <==
\section{Introduction}


% The need for energy-efficiency from {edge} to cloud computing has boosted the widespread adoption~of~FPGAs~\cite{diamantopoulos2018ectalk,kara2018columnml, dai2017foregraph}. {An FPGA is highly configurable as its circuitry can be tailored to perform any task. The massive configuration space and complex interactions among configuration options lead many 
% {developers} to explore individual optimization options in an ad-hoc manner.  Therefore, developing an efficient FPGA accelerator %and finding the right system configuration for it (e.g., IBM CAPI offers three versions of cache-coherent interconnects) 
% requires tremendous engineering effort. Moreover, FPGAs have infamously low productivity due to the time-consuming FPGA {implementation} process.
% Exploring the high-dimensional design space can take hours or even days.   
% A common challenge that past works {face} is how to evaluate the performance of an FPGA implementation in a reasonable amount of time~\cite{mutlu2019}. }
%-------------------------------------------------------------------------------
%Power consumption has become one of the significant bottlenecks for our current computer systems. To overcome this issue, complementing general-purpose cores with specialized FPGA accelerators is a promising approach to enhance overall system performance without a significant increase in power consumption. 
The need for energy efficiency \om{and flexible acceleration of workloads} has boosted the widespread adoption of field-programmable gate arrays (FPGAs)~\cite{singh2021fpga,van2019coherently,singh2019narmada,singh2019low} \om{in both edge and cloud computing}. Past works~\cite{singh2021fpga,van2019coherently,singh2019narmada,singh2019low,jiang2020boyi,cali2022segram, dai2017foregraph,alser2017,alser2019sneakysnake,diamantopoulos2018ectalk,kara2018columnml,singh2022accelerating} show that FPGAs can be employed {effectively} \om{to accelerate} a wide range of applications, {including graph processing, databases, neural networks, %{and} 
weather forecasting, \juang{and genome analysis}}. 
%In addition to the reconfigurability of an FPGA to implement diverse workloads, FPGA's flexibility in a cloud system is attributed to its cloud deployment model~\cite{arefmicrosoft,choi2019depth,aws,alibaba,pourhabibi2020optimus,byma2014fpgas,singh2020nero,singh2019low, singh2019narmada,singh2021fpga,singh2022accelerating,van2019coherently}. %These deployment models span from on-premises clusters to compute, storage, and networking capacity in public clouds.
% {In cloud computing~\cite{arefmicrosoft,choi2019depth,aws,alibaba,pourhabibi2020optimus,byma2014fpgas}, %era, 
% FPGA's flexibility is attributed to  % \jgl{Do not start the sentence like that. It sounds as if you had talk about FPGA flexibility before.} is not just about being able to make use of reconfigurable hardware for a diverse set of workloads~\cite{10.5555/3294624}. {Its flexibility can also be 
% attributed to the}  {cloud} deployment model that spans from on-premises clusters to compute, storage, and networking capacity in public clouds, %and even out to the edge \jgl{The edge? Aren't we talking about FPGAs in the cloud?} 
% where AI and analytics are being increasingly deployed because of latency and data movement issues~\cite{mutlu2019} \jgl{This sentence can be better two clearer sentences.}.} 
% that combine CPUs with specialized accelerators, GPUs, and/or FPGAs. 
% Complementing general-purpose CPU cores with FPGAs~is a successful approach because of the reconfigurability and energy efficiency of FPGAs. 

%  However, taking full advantage of an FPGA for accelerating a workload is not a trivial task.
% First, FPGAs run at extremely low frequencies compared to the state-of-the-art CPU. Therefore, to match the CPU's performance, an FPGA must exploit at least one order of magnitude more parallelism in a target workload. Second, efficient FPGA designing requires comprehensive knowledge of the FPGA micro-architecture with sufficient FPGA programming skills, which often leads to a significant design effort. Third, CPU and FPGA are connected via low-bandwidth I/O links, which cause significant data movement overhead. 


An FPGA is highly configurable as its circuitry can be tailored to perform any task. \om{However, FPGA developers face two main issues while \juang{designing} an accelerator.} % However, an efficient {implementation of a workload on an} FPGA requires comprehensive knowledge of the FPGA {microarchitecture} combined with sufficient FPGA programming skills. 
%  From a systems perspective, the design choices {are made more complex} by various interconnect options, such as upcoming %high-bandwidth} 
%  interconnect technologies from IBM CAPI~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators
% (CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{sharma2019compute}.
%This often leads to a significant design effort. 
\om{First, the} large configuration space of \om{an} FPGA and {the} complex interactions among \om{its} configuration options \om{cause} many 
developers to explore optimization \om{techniques} in an ad-hoc manner~\cite{diamantopoulos2020agile,singh2021modeling}. 
\om{Second, FPGA programming leads to low productivity because of the time-consuming accelerator design and implementation} process~\cite{o2018predictive}. 
%Exploring the high-dimensional design space can take hours or even days.   
Therefore, a common challenge that past works {have faced} is how to evaluate the performance \juang{(and resource \omm{usage})} of an accelerator implementation in a reasonable amount of time~\cite{o2018hlspredict}. 
 %{The development of efficient FPGA accelerators has, thus, required tremendous engineering effort due to the complexity of the FPGA configuration space and difficulties in evaluating performance. }
 %Therefore, developing an efficient FPGA accelerator %and finding the right system configuration for it (e.g., IBM CAPI offers three versions of cache-coherent interconnects) 
%requires tremendous engineering effort.
To overcome this problem, researchers have {recently} employed machine learning (ML)-based models~\cite{makrani2019pyramid,ferianc2020improving,ustun2020accurate,o2018hlspredict,xppe_asp_dac,dai2018fast,zhao2019machine,yanghua2016improving,wang2020machine,mahapatra2014machine,singh2019napel} to \om{%evaluate an
\juang{predict the performance and resource \ommm{usage} of a given} accelerator implementation quickly. %}{estimate}  the performance of an FPGA-based system quickly. 
% These models are} based, in turn, on traditional ML {approaches}. %\juan{(e.g., give examples...)}. 
However, these ML-based models have three fundamental issues that %reduces the usability of such approaches.
\juang{reduce their usability.}}% assessing FPGA performance, especially in a cloud system}. 

First, \om{these ML-based} %approaches} 
\juang{predictors} are trained for specific workloads, fixed hardware, and/or a set of inputs. {Therefore,} we cannot reuse these models for %when presented with a different feature-space distribution 
\juang{a} \om{previously \textit{unseen}} workload or \om{a different FPGA platform} because the trained model does not have a notion of the new, {unknown} environment.\footnote{We consider a new workload or a \omm{new} FPGA platform as a \omm{new} environment.} %, {an ML model must} be \gs{fine-tuned or} retrained from scratch. Otherwise, {the model} will perform poorly because the trained model does not have a notion of the new, {unknown} environment.\footnote{We consider a new workload or hardware as an environment.} %\footnote{{In this paper, we consider an application or hardware platform as an environment.}} 
Therefore, traditional ML-based models have limited \textit{reusability}.

Second, \om{ML-based models} require a %considerable 
\omu{large} {number} of samples to construct a useful \om{performance} predict\om{or}. Collecting such a large number of samples is often \om{very} time-consuming due to the very long \om{accelerator} implementation cycle \om{on an FPGA, especially in a cloud computing environment \omu{where} data collection could be costly.} % \jgl{Check Onur's comment.}
% Similarly,  collecting enough samples in %settings such as cloud computing
% cloud computing \om{environmen is often \textit{infeasible} because of its \textit{cost} and \textit{error-prone} behaviour.} % \jgl{Again, clarify error-prone and infeasible.}, the data collection process is even more difficult. \jgl{FPGA design cycle is time-consuming and error-prone + cloud is expensive = collecting enough samples is (almost) infeasible.}

Third, \om{ML-based} models trained using a limited \juang{number of} samples are prone to serious \emph{overfitting} problems \juan{(i.e., model matches to the training data \om{too closely)}}~\cite{dai2007boosting}, limiting model generalization. %\om{to adapt properly to new, previously unseen data}. %\jgl{I think this one would go better as "Second".}


%This 
% Our research aims to answer the following question: for an FPGA-based system, can we leverage and transfer our ML-based performance models trained on a low-end local system to a new, unknown, high-end FPGA-based system, thereby avoiding the limitations of traditional ML-based approaches
\textbf{Our goal} is \juang{to overcome these three issues of ML-based models for prediction of FPGA performance and resource \ommm{usage}.} 
\juang{To this end, we present \namePaper. Our key idea is} 
to leverage an ML-based performance and resource \ommm{usage} model trained for a low-end \om{edge environment} to predict performance and resource \ommm{usage} of an accelerator implementation \om{for a new, high-end cloud environment.} %, thereby avoiding the limitations of current ML-based models.} 
%\om{for a: 1) new, high-end cloud environment, or 2) new application,} thereby avoiding the limitations of current ML-based models.
% \textbf{Our research aims to answer the following question: for an FPGA-based system, can we leverage an ML-based performance model trained on a low-end local system to predict the performance in a new, unknown, high-end FPGA-based system?}%. 
% \jgl{I do not like the question. I prefer a clear statement of the goal/s.}
% \jgl{There is repeated text in this paragraph.}
% \jgl{We haven't talk about transfer learning yet. It is better to just ask something like: "Is there a way to leverage an ML-model trained for a specific low-end environment to predict the performance in an unknown high-end environment?" Then, we can talk about transfer learning in the introduction to Leaper.} 
%To this end, 

%{To this end,} we present 
\namePaper\footnote{We call our mechanism \namePaper~because it allows us to hop or ``leap'' between machine learning models.} \juang{employs} a transfer learning-based approach 
%to predict performance and resource utilization of \om{an accelerator implementation for} a new, high-end cloud FPGA-based system or a new application on the same FPGA-based system. 
\juang{(also called \textit{few-shot learning}~\cite{fsl}). 
This technique is based on the idea that algorithms, similar to humans, can learn from past experiences and \emph{transfer} knowledge to the resolution of previously-unknown tasks.} 
\juang{Concretely, \namePaper transfers an ML-based model trained on an edge FPGA-based system to a new, high-end cloud FPGA-based system.} 
\gs{Using an edge FPGA-based system for %training data collection has three major benefits compared to using an high-end cloud FPGA-based system. 
\juang{training the ML-based model provides three major benefits over using a high-end FPGA.} 
First, since %the 
edge devices are small, FPGA bitstream generation is faster compared to generating bitstream for a high-end FPGA. 
Second, edge FPGAs are cheaper and more affordable. 
Third, a high-end FPGA often requires integration with a server-grade host CPU, which can be %cost-prohibitive or even inaccessible 
\juang{costly or not possible} for many users. 
Therefore, using low-cost and broadly available edge systems for \juang{training} data collection can} %provide fast turnaround time.}  
\juang{greatly facilitate the generation of ML-based predictors for performance and resource \ommm{usage} of FPGA-based systems.} 
% \namePaper helps a user to rapidly quantify such a decision by experimenting with low-cost and broadly available FPGAs, like the PYNQ-Z1.

%Transfer learning is also referred to as \textit{few-shot learning}~\cite{fsl}. The idea behind {few-shot learning} is that, similar to humans, algorithms can learn from past experiences and transfer the knowledge to accomplish previously-{unknown} tasks more efficiently. %The transferred models usually have high generality~\cite{fsl}. 
%\jgl{We also use LEAPER for transferring models across applications, right? We should also say that here.}
%uses three main steps to transfer an ML-based performance or resource utilization model. 
\juang{\namePaper consists of three main steps.} 
\juan{First,} \namePaper uses \emph{design of experiments} (\emph{DoE})~\cite{montgomery2017design}, \juang{a technique} to extract representative \juang{training} data %with 
\juang{from} a small number of experimental runs. %from a low-end edge environment. %using which we built 
%The goal of transfer learning is 
\juan{Second,} %we train 
\juang{\namePaper trains} an ML-based model (\textit{base model}) to predict performance or resource \ommm{usage} for an accelerator implementation on a low-end edge environment. 
\juan{Third,} 
%uses \emph{transfer learning} to %leverage \juan{efficiently adapt the} 
\juang{\namePaper transfers the} 
trained base model %(for a low-end system) adapt it efficiently 
to %\om{predict performance or resource utilization for an accelerator implementation for} 
a new, high-end \emph{cloud} environment (a new FPGA or a new application) with only a few \juang{new training samples (between 5 to 10 samples) from the new environment}. %{\namePaper also transfers a model across unknown, new applications implemented on the same FPGA-based platform.} 


Figure~\ref{fig:transfer_intro} compares the traditional ML-based approach (\circled{a}) to \namePaper  (\circled{b}). Using the traditional ML-based approach, we would %have 
\juan{need} to create two separate prediction models, \juan{one} for the \juan{low-end} edge \juan{environment} and \juan{another one for the high-end} cloud environment, each \juan{one} requiring a large number of samples. \namePaper transfers a previously trained model to a new, unknown environment using transfer learning with only a few training samples. 
%\namePaper allows transfer of models from a low-cost edge FPGA, where data collection is easier, to a high-cost cloud FPGA environment to build cheaper and faster models using transfere learning.

 \begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth,trim={0.2cm 0.45cm 0.4cm 0.3cm},clip]{images/Transfer_intro_cr_4.pdf}
    % \caption{Transfer learning from low-cost edge FPGA to a high-cost cloud FPGA environment}
    %  \vspace{-0.3cm}
  \caption{Traditional ML-based approach vs. \namePaper.} % {Traditional learning methods are costly because they build models only for a specific environment. } LEAPER allows transfer of models from a low-cost edge FPGA, where data collection is easier, to a high-cost cloud FPGA environment to build cheaper and faster models.}
  \label{fig:transfer_intro}
 \end{figure}
 \vspace{0.1cm}
% Fourth, it is humanly impossible to {construct} one model for all different scenarios. \jgl{Better remove this one...}
% Fourth, it is impossible to {construct} one model for all different scenarios as the interpretation of data changes over time. Thus, ML models are prone to \emph{concept drift}, where the accuracy of an ML-based model could degrade due to change in the statistical properties of a target variable \juan{(e.g., using a different dataset for an application than the one used during the training of an ML-model)}~\cite{model_drift}.


% {\textit{Transfer learning~\cite{pan2009survey}} \jgl{Cannot start like that. First, say what is Leaper, then say that Leaper uses transfer learning.} allows us} to leverage a trained \textit{base model} \juan{(for a low-end system)} and adapt it efficiently to an unknown, \emph{\juan{target}} environment \juan{(i.e., a high-end system)} with as few samples from the target environment as possible. 



% Figure~\ref{fig:transfer_intro} also shows the \namePaper transfer learning-based approach.  %\jgl{To me, the previous sentence is motivation and we should refer to this part of the figure before stating the goal}. 
% In contrast to the traditional approach, \namePaper~provides the ability to reuse the prediction model  built on an {\emph{inexpensive}} edge FPGA for {performance prediction on a target} cloud environment~\footnote{Note: LEAPER is not limited to a cloud environment. \jgl{Unnecessary footnote?}} using only a few samples \juan{from the target environment}. 
% {This allows \juan{developers} to avoid the slow downstream implementation process of FPGAs %to develop
% \juan{by generating} cheaper and faster performance models} using transfer learning \jgl{We knew this already. Too much repetition. The right part of Figure 1 can be directly explained at the end of the previous paragraph. The left part of Figure 1 should be explained in the motivation (before the goal).}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {\namePaper~builds} ML models that predict %the
% performance %/
% and resource usage for an application {on an FPGA}. With \textit{few-shot learning}, it adapts these models to a new, unknown environment, %{(i.e., a new FPGA or a new application)} %for 
% {from} which only a few labeled samples are %available.
% {needed}. {\namePaper~uses a statistical} technique called \textit{design-of-experiments} to collect the training data. This technique aims to cover the entire design space effectively in a limited {number of} experimental runs~\cite{singh2019napel}. We use \textit{Latin hypercube sampling} (LHS)~\cite{LHS} to sample FPGA's high-dimensional configuration
% space judiciously. The conventional brute-force approach to run every single input configuration on all the chosen platforms quickly becomes impractical. This is due to the large design space, combined with {the} long FPGA runtime (1-12 hours for a single point), which may take months or years~\cite{liu2013learning}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {Works, such as~\cite{singh2019napel,li2018processor,liu2013learning} show the effective use of these approaches.} 
% in this paper, we apply a 

% Howerver, to collect training data for all these scenarios will lead to massive space. The FPGA allows us to have plethora of optimization options. Moreover, if you want to make your ML model cross platform you execute all these combinations on different FPGA devices. 

% In traditional {ML} approaches, researchers exhaustively run every single input configuration on all the chosen platforms to collect the training data~\cite{tulikaML}. 
% The considerable design space, combined with {the} long FPGA runtime (1-12 hours for a single point), may take months or years~\cite{liu2013learning}, which makes the traditional exhaustive approach impractical. 
% %This calls for 
% {To overcome this issue, we use} %some 
% statistical techniques {to} effectively cover the entire design-space in a limited {number of} experimental runs~\cite{singh2019napel}. 
% % {Works, such as~\cite{singh2019napel,li2018processor,liu2013learning} show the effective use of these approaches.} 
% % in this paper, we apply a 
% {\namePaper~applies a statistical} technique called \textit{design-of-experiment} (DoE).  Specifically, we use \textit{latin hypercube sampling} (LHS)~\cite{LHS} to sample the high-dimensional configuration
% space wisely.
% To address this issue, we need to derive a robust
% prediction model by sampling which motivated us to propose a novel transfer learning based model and a weighted LHS sampling method.


% To find the right applicaiton input we need to perform input sensitivity analysis~\cite{Autotuning algorithmic choice for input sensitivity}. This entails extracting domain-specific algorithmic choices that influence the FPGA design, which inturn affect the overall performance. The large number of inputs, comined with long FPGA run-time (4-8hours for a single point) may take months or years, which makes the traditional exhuastive approach impratical.
\gs{
\head{Key results} We demonstrate \omm{\namePaper} across \textit{five} {state-of-the-art,} high-end, cloud FPGA-based platforms with \textit{three} different {interconnect} technologies on \textit{six} real-world applications. %{The kernels are specified in C/C++ and compiled to the FPGA target using Vivado HLS for the target and Xilinx SDSoC for the base model.}
We \omm{present} two keys results.
First, \namePaper achieves, on average \omm{across six evaluated workloads and five FPGAs, 85\% accuracy when we use use our transferred model for prediction in a cloud environment}. Second, \namePaper~\ommm{greatly} reduces (up to 10$\times$) the training overhead by \omm{transferring} a \textit{base model}, trained %\om{to predict performance or resource utilization for an accelerator implementation} 
for a low-end, {edge} {FPGA} platform, \om{to predict performance or resource \ommm{usage} for an accelerator implementation} on a {new}, unknown high-end environment rather than building a new model from scratch. %(Section~\ref{subsection:timing}).
}

This work makes the following \textbf{major contributions}:

%\vspace{-0.1cm}
\begin{enumerate}

\item We \ommm{introduce} \namePaper, \omm{a \ommm{new} transfer learning-based framework for prediction of performance and resource \ommm{usage} in FPGA-based systems.} %to transfer FPGA-based \gs{performance and resource utilization} models across different hardware platforms and applications. 

\item Unlike state-of-the-art works~\cite{makrani2019pyramid,ferianc2020improving,ustun2020accurate,o2018hlspredict,xppe_asp_dac,dai2018fast,zhao2019machine}  in FPGA modeling that use deep neural networks, we show that classic non-neural network-based models are enough to build an accurate predictor to evaluate an accelerator implementation on an FPGA.


% \item We design an \emph{ensemble transfer learning model} based on the \textit{boosting} and \textit{Bayesian process} that transfers accurate models to a new target environment with few learning samples (Section~\ref{subsec:ensemble_transfer}). 
%\jgl{Isn't this the same as 1) with different words? {I was thinking more like that we have ensemble of learners (two learners)}}

% \item We reduce the time needed to gather
% data for {model training} by employing a \textit{design-of-experiments} technique (Section~\ref{subsec:lhs}), which
% selects a small number of input configurations
% that represents the entire space of input configurations.
% \item We create an {ensemble of transfer learning models} to transfer learning from multiple base learners accurately to avoid a negative transfer, i.e., a severe degradation of the predictive power of the transferred model (Section~\ref{subsec:ensemble_transfer}). % The use of {multiple} base learners lets us avoid severe degradation of the \textit{transferred} model's predictive power, i.e., avoid a \textit{negative transfer} \jgl{What is a negative transfer? If you want to include this term, then flip the sentence: "...to avoid a negative transfer, i.e., a severe degradation of the predictive power of the transferred model.}.  
\item We conduct an in-depth evaluation of \namePaper on real cloud systems with
various FPGA configurations, showing that \namePaper can develop cheaper, faster, and highly accurate models.
% \item We demonstrate our approach across \textit{five} {state-of-the-art,} high-end, {on-premise cloud} FPGA-based platforms with \textit{three} different {interconnect} technologies on \textit{six} real-world applications (Section~\ref{sec:evaluation}). %{The kernels are specified in C/C++ and compiled to the FPGA target using Vivado HLS for the target and Xilinx SDSoC for the base model.}
% For \textit{5-shot} learning, we achieve an average accuracy of 80--90\% for performance and resource utilization models. \namePaper dramatically reduces (up to $10\times$) the training overhead by adapting a \textit{base model}, trained on a low-end, {edge} {FPGA} platform to a {new}, unknown high-end environment ({a cloud environment in our case}) rather than building a new model from scratch (Section~\ref{subsection:timing}).
\end{enumerate}

==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/methodology.tex <==
\section{\namePaper}
\label{sec:methodology}

\namePaper~is a performance %/
{and} resource estimation %approach 
{framework} to \textit{transfer} ML models~\cite{swain1977decision,breiman2001random} across: \gs{(1) different FPGA-based platforms for a single application, and (2) different applications on the same platform.} In this section, we describe the main components of the framework.
%\jgl{Why don't you mention same platform, different apps here?}. 
First, we give an overview of \namePaper~(Section~\ref{subsec:overview}). Second, we describe the target cloud FPGA-based platform (Section~\ref{subsec:system}). Third, we discuss  accelerator optimization options and application features used for training an ML model (Section~\ref{subsec:fpga_deploy}). Fourth, we briefly describe the {base} model building (Section~\ref{subsec:base_model}).  Fifth, we explain the %important 
 {key} component of \namePaper to build cloud models:
 the transfer learning technique (Section~\ref{subsec:ensemble_transfer}). Sixth, we describe \namePaper's transfer learning algorithm (Section~\ref{subsec:transfer_algo}).
 
\subsection{Overview}
\label{subsec:overview}
% \namePaper~is based on transfer learning.  It~transfers a base model, trained on an \gaganT{inexpensive}, low-end source environment, to a new, {unknown}, high-end {cloud} environment through {few-shot learning}. 
%Similar to humans, \namePaper~learns from previous models rather than running every single application and FPGA design configuration on a new, {unknown} environment.
Figure~\ref{fig:transfer_overiew} \gs{shows} the key components of \namePaper % \jgl{Place the figure at the bottom of this page.}
. It consists of two parts: (1) base model building (low-end environment) and (2) target model building (high-end environment). %{The upper part of the figure describes the base model building, while the lower part shows the target model building.}
% We considered random forest and gradient boosting as our base statistical model, which has proven to be a robust feature-based model in past problems. 

 \begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth,trim={0.2cm 0.8cm 0.4cm 0.2cm},clip]{images/model_big_cr_3.pdf}
    %  \vspace{-0.1cm}
  \caption{Overview of %our approach
 \namePaper. %Base Model Building: {\namePaper~builds} ML models that predict %the
% performance %/
% and resource usage for an FPGA environment. Target Model Building: with \textit{few-shot learning}, \namePaper~adapts base models to a new, unknown environment, %{(i.e., a new FPGA or a new application)} %for 
% {from} which only a few labeled samples are %available.
% {needed}.
}
  \label{fig:transfer_overiew}
 \end{figure}
\noindent \textbf{Base model building.} \namePaper's base model building consists of three phases. The first phase (\circled{1} in Figure~\ref{fig:transfer_overiew}) is an LLVM-based~\cite{llvm} kernel {analysis} phase (Section~\ref{subsec:fpga_deploy}), which extracts architecture-independent workload characteristics.  We characterize in a microarchitecture-independent manner by using a specialized plugin of the LLVM compiler framework~\cite{Anghel2016}. This type of  characterization excludes any hardware dependence and captures the inherent {characteristics} of workloads.

In the second phase~\circled{2}, we generate accelerator implementations to gather accelerator \omu{implementation responses \ommm{(performance and resource utilization)}} for training. Once the accelerator design has been implemented, the {resulting FPGA-based} accelerator is deployed {in a system} with a host CPU. %system. %Following which 
We employ the \emph{design of experiments}  (DoE) technique~\cite{montgomery2017design}
%\textit{Latin hypercube sampling} (LHS)~\cite{li2018processor} %is first employed 
to select a small set of accelerator optimization configurations that well represent the entire space of accelerator optimization configurations ($c_{doe}$) to build a highly accurate \textit{base learner}. 
%We use DoE to minimize 
\juan{By using DoE, we minimize} the number of experiments needed to gather training data for \namePaper~while ensuring {good} quality training data. %(Section~\ref{subsec:lhs}). 
{Then,} we %use 
{run} {the} $c_{doe}$ configurations on %an FPGA-based platform 
{the deployed FPGA-based system} to gather samples % \jgl{samples? We haven't defined what we mean by response.} 
for training our base model. The generated responses along with application properties from the first phase and the accelerator optimization parameters form the input to our base learner.
In the third phase~\circled{3}, we train our base learner (Section~\ref{subsec:base_model}) using ensemble learning~\cite{opitz1999popular}. %that uses both \textit{boosting} and \textit{bagging}-based ML techniques to create a robust ensemble model. 
%During this phase, we perform 10-fold cross-validation to validate the performance of our model. %During cross-validation, we divide our dataset into 10 equal subsamples of which 1 set is used for validation. % \jgl{What is a 10-fold cross-validation?}. 
During this phase, we perform additional tuning of our ML algorithm's hyper-parameters.\footnote{Hyper-parameters are sets of ML algorithm variables that can be tuned to optimize the accuracy of the prediction model.}  
Once trained, the framework can predict the performance and resource usage {on the base environment (a low-end edge system)} of %all 
{previously-unseen} configurations, %that 
{which} are not part of the $c_{doe}$ {configurations used during the training.} %{on the base system, i.e., the low-end FPGA}.

\begin{figure*}[h]
\centering
\begin{subfigure}[h]{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/cr_System1.pdf}
  \vspace{-1.2cm}
  \caption{
  \label{fig:system}}
\end{subfigure}%
\hspace{0.7cm}
\begin{subfigure}[h]{.3\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/cr_Execution_timeline_1.pdf}
%   \vspace{-0.5cm}
\vspace{-1.2cm}
   \caption{ \hspace{-6.2cm}
  \label{fig:execution}}
\end{subfigure}
%  \vspace{-0.2cm}
\caption{(a) Experimental cloud platform: High-end cloud FPGA platform with IBM\textsuperscript{\textregistered} POWER9  CPU. %FPGA acts as a peer to the  CPU by accessing the main-memory~through a high-performance CAPI link, enabled by Power Service Layer (PSL). {A processing element (PE) is composed of basic~FPGA~components i.e., CLB, BRAM, and DSP.} 
(b)  Execution timeline with data flow sequence from the  host to the FPGA.} %A software-defined API handles %offloading jobs 
% job-offloading to PEs with an interrupt-based queuing mechanism.
 %\label{fig:system}}
% \vspace{-0.4cm}
\end{figure*}
\noindent \textbf{Target model building.} %We use  transfer learning to reuse an ML model (trained on a low-end FPGA) in a high-end cloud environment. 
\gs{\namePaper's target model building consists of three phases.} 
%{To transfer the base model, which we built in the previous stage, to a target cloud environment, we introduce the \emph{few-shot learning} target model stage.} 
The first and the second phase\ommm{s} (\circled{A} and \circled{B} {in Figure~\ref{fig:transfer_overiew}}) \ommm{are} the same LLVM-based kernel analysis and the accelerator generation phases as in base model building, respectively. %} is the same accelerator \jgl{Is it the same accelerator? Need to say that this is repeating the phase on the high-end FPGA to get the few samples.} generation and deployment phase as in the base model building stage
We perform this step to create our \textit{few-shot}  learning dataset ($c_{tl}$), % and transfer learning test set ($c_{lhs}$-$c_{tl}$). 
 which is used to adapt the low-end edge model to the target cloud environment.\footnote{We show \ommm{via} experiments (Section~\ref{sec:result}) that up to 5 samples (\emph{5-shot}) are enough to learn the \ommm{characteristics} of a new environment.} 
% To create $c_{tl}$, in the second phase \circled{B}, we perform subsampling of $c_{lhs}$ \jgl{For what?}. 
In the final phase \circled{C}, we train our ensemble transfer learner (Section~\ref{subsec:ensemble_transfer}) to leverage the low-end edge model to perform predictions for a new target environment (new application or FPGA). %\jgl{New application? We are not talking about new applications! Either we talk about new applications from the beginning of the paper, or we don't talk about them (and only in the evaluation we say "Oh, btw, Leaper also works for new applications on the same platform!".}
 %to leverage the base model to perform predictions of a new target environment (new application or hardware). 
% We show by empirical experiments, rather than running every single application and FPGA design configuration on a new platform, we can leverage the previously built model through transfer learning.  

\subsection{Target Cloud FPGA-based Platform}
\label{subsec:system}

\gs{Figure~\ref{fig:system} shows the high-level overview of our  FPGA-based cloud  platform. An FPGA is connected to a server system
based on an IBM POWER9 processor using the Coherent Accelerator Processor Interface  (CAPI)~\cite{stuecheli2015capi}. Our
design consists of multiple processing elements (PEs) that
interact with the host system through the power service
layer (PSL), which is the CAPI endpoint on the FPGA. A PE can utilize the on-chip FPGA elements such as  DSP (digital signal processor), CLB (configurable logic block)\footnote{CLB is the fundamental component of an FPGA, made up of look-up-tables (LUTs) and flip-flops (FF).}, and BRAM (block RAM) to implement an application.}

Figure~\ref{fig:execution} shows the execution timeline from our host CPU to the FPGA board. We make use of CAPI in a coarse-grained way as we offload the entire application to the FPGA. CAPI ensures that a PE accesses the entire CPU memory with the minimum number of memory copies between the host and the FPGA, e.g., avoiding the intermediate buffer copies that  traditional PCIe-based DMA invokes~\cite{10.1145/2897937.2897972,singh2020nero}. However, depending on the application, the CAPI protocol can be employed in a fine-grained algorithm-hardware co-design, like in  \textit{ExtraV} \cite{extraVLee2018VLDB}, \omu{which exploits} the fine-grained communication capability of CAPI. On task completion, the PE notifies the host CPU via the AXI lite interface~\cite{axilite} and transfers back the results via CAPI-supported DMA transactions.



% \subsection{Accelerator  Optimization Options and Application Features}
\subsection{Application Features and Accelerator  Optimization Options}
\label{subsec:fpga_deploy}
The ML feature vector used for training our base and target models is composed of two parts: application features and accelerator optimization options.


\noindent \juan{\textbf{Application features.}}
{We include inherent application features in our training dataset.}
{For each application kernel \textit{k} processing a dataset \textit{d}, we obtain an application profile \textit{p(k, d)}.} 
\textit{p(k, d)} is a vector where each parameter is a statistic about an application feature. 
Table~\ref{tab:application_features} lists the main application features {we extract} {by using the LLVM-based PISA analysis tool~\cite{Anghel2016}}. Ultimately, the application profile \textit{p} has 395 features, which includes all the sub-features %\jgl{What are the subfeatures? Have you introduced them? In Table 2, I only see features, not subfeatures.} 
{of each metric we consider}.
{We perform feature selection to select} the 100 most important features to analyze the behavior of an application. % with the FPGA configuration options (see Table~\ref{tab:pragma}). 
% \jgl{At this point, if the reader is paying attention, he/she will understand that the ML feature vector used for training is composed of values for the features in Table 1 and Table 2. The problem is that we are not saying this anywhere. This should be the first thing to say in the beginning of 2.3.}

\input{tables/metrics.tex}

\noindent \juan{\textbf{Accelerator optimization options.}}
Table~\ref{tab:pragma} describes commonly used high-level synthesis (HLS)~\cite{hls} pragmas to optimize an accelerator design on an FPGA. These optimization options constitute a part of our ML feature vector for training. %\gs{These pragmas represent the most commonly used optimization directives  that can have significant performance impact while tuning an FPGA implementation.} %These configuration options among the features because of their large potential impact on performance.  % {We select these HLS pragmas because they are used to optimize and tune the performance of FPGA implementations~\cite{xilinx_hls_guide}.}
We use eight optimization options. First, \textit{loop pipelining} {(PL)} optimizes a loop to overlap different loop operations. Second,  \textit{loop unrolling} {(UR)} creates multiple copies of a loop for parallel execution. PL and UR aim to increase the processing throughput of an accelerator implementation.
%Both \textit{loop pipelining} {(PL)} and \textit{loop unrolling} {(U)} can improve application performance significantly. %\jgl{Completely empty sentence. Do you want to say that you include them among the features because of their large potential impact on performance? You can also say that they are widely used or among best practices, and cite something.}. %Memory operations are often the performance bottleneck in real applications. 
Third, to enable simultaneous memory accesses, \textit{array partitioning} {(PR)} divides \ommm{an} array into smaller units of \ommm{desired partitioning factor} %by carefully deciding how 
and maps {them} %arrays 
to %memories has a significant influence on the overall implementation
{different memory banks.} This optimization produces considerable speedups but consumes more resources. Fourth, \textit{inlining} {(IL)} ensures that a function is instantiated as dedicated hardware core. Fifth,  \textit{dataflow} {(DF)} optimization exploits task-level parallelism to allow parallel execution of tasks. %, which is similar to multi-threading in CPUs. % \jgl{if multithreading exploits task level parallelism...}. 
%In addition, we take advantage of the large FPGA area to \textit{replicate} accelerators. 
Sixth, \textit{burst read} {(BR)} controls burst reads from the host to the accelerator. Seventh, \textit{burst writes} {(BW)} controls burst write to the host from an accelerator. Eighth, \textit{FPGA frequency} {(FR)} constrains an accelerator implementation to a specific clock frequency. It affects {not only} the performance %and 
{but also} the resource \ommm{usage of} an implementation. For instance, to meet the FPGA timing requirements, the FPGA tool inserts registers between flip-flops, {which increases  resource \ommm{usage}}. 

\input{tables/pragma_configuration.tex}

In total, our optimization options {for a particular application} leads {up to} 4,608 configurations. However, the actual optimization space of an application depends %indirectly 
on the specific application characteristics (see Table~\ref{tab:app_details}). %, e.g., 
{For example, we include} loop unrolling {in the optimization space when an application contains loops that can be unrolled.}  %{Note:  Table~\ref{tab:pragma} describes the configuration options used to train our ML-models.} 
%is effective only when an application’s loop can benefit from it.





% \jgl{The organization is not good. We talk about LHS in 2.2. before talking about the FPGA configuration options in 2.3. Better organization is: 1) Section 2.2 talks about FPGA configuration options, including LHS; 2) Section 2.3 talks about application features.}
% \subsection{Latin Hypercube Statistical Sampling}
% \label{subsec:lhs}
% \subsection{Design of Experiments Technique}
% \label{subsec:lhs}
% %It would be imprudent to exhaustively run for all the available optimization options, which is often done in research to collect training data. 
% {Running experiments to collect training data for all available optimization options can be an extremely time-consuming process. For example,} 
% the configuration options ($\mathbb{CO}$) of %just 
% {only} eight parameters {with two possible values each,} %, even with binary options, would lead to
% {entails} $2^8=256$ different configuration inputs. 
% If we spend 6 hours (e.g., FPGA downstream implementation process on an ADM-PCIE-KU3 {FPGA board}~\cite{adku3}) to collect one training point, it would take {us} %$\approx$
% $\sim$64 days to collect data for all configurations %options 
% for just \textit{one} application on a \textit{single} platform. 
% {This ``brute-force'' approach to collecting training data is too time-consuming: the sheer number of experiments renders {a} detailed implementation intractable}.

% To create a %cost-aware 
% {cost-effective} model, we use the {\emph{design of experiments} (DoE) methodology}~\cite{montgomery2017design} %method
% to minimize the number of experiments needed %to train
% {for training data collection}, without sacrificing the amount and quality of the information gathered %by 
% {from} the experiments. 
% DoE is a set of statistical techniques meant to locate a small set of points in  parameter space to represent the entire parameter space.
% %The traditional brute-force approach to collecting training data is {too} time-consuming: the sheer number of experiments renders detailed simulations intractable. 
% %Thus, the DoE strategy to gather a training dataset is a critical component of our model. 
% % {In particular, we make use of {a type of DoE called}  \textit{Latin hypercube sampling} (LHS)~\cite{li2018processor} because it allows each of the critical parameters to be represented in a fully stratified manner (i.e., dividing the configuration space into subgroup before further sampling), which provides a better coverage~\cite{fang2002centered}.}
% LHS divides each parameter range into \textit{k} intervals and takes only one sample from each interval with equal probability, which is more efficient than a random approach and more cost-effective than a ``brute-force'' approach. % \jgl{I would say it "is more efficient than a random approach and more cost-effective than a brute-force approach".}.
% To apply %Latin Hypercube sampling, one must
% {LHS, we} %first 
% choose \textit{m} sample points, each from a specific interval,  which together we refer to as \textit{c$_{lhs}$} % \jgl{Not clear: \textit{c$_{lhs}$} is a configuration point, which considers multiple parameters; but when we talk about intervals above, we talk about each parameter.}. %; hence 
% {Thus,} LHS guarantees effective space-filling i.e.,  LHS spreads out points with the aim of encouraging a diversity of data~\cite{li2018processor}. %\jgl{One can guess what "space-filling" is, but it is just a fancy term for free... Let's explain fancy terms if we use them.}.  
% Figure~\ref{fig:LHS} illustrates LHS with two parameters {\textit{x1} and \textit{x2}}, %where the 
% {which create an} input space {that} is divided into equal {area} intervals. %{To select the amount of samples to build a precise performance prediction model we follow the approach from Valov~\etal~\cite{valov2015empirical} \jgl{And this approach consists of what?}.}   %We use T\textit{$\times\mathbb{CO}$} samples, where T=5 allows to build highly accurate prediction models.

% % \input{images/LHS.tex}



\subsection{Base Learner Training}
\label{subsec:base_model}

The third phase of base model training is the training of the base learners. We use {an \emph{ensemble} of} two \gs{non-linear} base learners \gs{that {can} capture the intricacies of accelerator implementation by predicting the execution time %or 
or the resource \ommm{usage}.} %of a {heterogeneous} CPU-FPGA platform.  
Our first algorithm is the \emph{random forest} (RF)~\cite{breiman2001random}, which is based on \emph{bagging}~\cite{breiman1996bagging}. %RF consists of an ensemble of learners where it aggregates the predictions of the weak learners to select the best prediction. This technique is called as \textit{bagging}. 
We use RF to avoid a complex feature-selection scheme % and moreover it} 
{since RF} embeds automatic procedures {that are able} to screen many input features~\cite{mariani2017predicting}. %{like the ones we selected in the previous section}. 
Starting from a root node, RF constructs a tree and iteratively grows the tree by associating %it 
{a node} with a splitting value for an input %variable 
{feature} to generate two child nodes. 
Each node is associated with a prediction of the target metric equal to the observed {mean} value in the training dataset for the input subspace that the node represents. 
Our second learner is \emph{gradient boosting}~\cite{gradientboosting}. %, which consists of an ensemble of learners. 
\gs{Gradient boosting aims to \textit{boost} {the accuracy of a weak learner} by using other learners to correct its predictions.}
Bagging~\cite{schapire1990strength} reduces model variance, and boosting decreases errors~\cite{kotsiantis2004combining}. Therefore, we use RF and gradient boosting together to increase the predictive power of our final trained base model.
%The third phase of the base model building is the base learner training phase. Formally,  
In a machine learning task, $\mathcal{X}$ represents \ommm{the} feature space with label $\mathcal{Y}$, where a machine learning model is responsible for estimating a function $f: \mathcal{X} \to \mathcal{Y}$. %we predict time
{\namePaper uses \textit{base learners} to predict the performance (or resource \ommm{usage}) $\mathcal{Y}$ for a tuple} \textit{(p, c)} {that belongs to the ML feature space $\mathcal{X}$}, where \textit{c} is \ommm{a set of} accelerator optimization options  %running
\ommm{for an} application profile \textit{p(k,~d)}.% by using \emph{base learners}.%, with %\textit{c} configuration for {an optimization configuration vector \textit{c}}. 

{The training dataset for our base model} has three parts: (1)  an application configuration vector \textit{p(k,~d)}, (2) an accelerator optimization option %pair
\textit{c}, and (3) responses corresponding to each pair \textit{(p, c)}.
To gather the accelerator responses, {we run each} application \textit{k} belonging to {the} training set $\mathbb{T}$ with {an} input dataset \textit{d} %is executed 
on an FPGA-based platform \ommm{while using an accelerator optimization \textit{c}}. 
%This produces time\textit{(p,~a,~d)} for that configuration and is used 
{This way, we obtain the execution time for the tuple \textit{(p, c)}, which we can use} 
as a \textit{label} ($\mathcal{Y}$) for training our base learner {for performance prediction}. 
%Similarly, we build another model 
{We build a similar model} to predict resource \ommm{usage}, where we use {the} resource \ommm{usage} ($\eta_{\{BRAM, FF, LUT,  DSP\}}$) {of the tuple \textit{(p(k,~d), c)}} as a \textit{label} when we train our base learner {for resource \ommm{usage}}. 
After \ommm{it is trained,} our base learner %algorithm, 
it can predict the {execution} time (or resource usage) ($\hat{f_s}:\mathcal{X}_s \to \mathcal{Y}_s$) of %configurations 
{tuples \textit{(p(k,~d), c)}} that are \emph{not} in the training set.

We improve base learner performance by tuning the algorithm’s hyper-parameters~\cite{scikit-learn}. Hyper-parameter tuning can provide better performance estimates for some applications. First, we perform as
many iterations of the cross-validation process as hyper-parameter
combinations. Second, we compare all the generated models by
evaluating them on the testing set, and select the best one.

 %, that forms a part of the ML feature space $\mathcal{X}$. 
% \jgl{If you want to use the formal definition, which is probably not necessary, start the section with it. Then, talk about the two learners. Then, talk about execution time and resource consumption. It seems there are different models for these two, but it is no clear from the text.}

%The input data gathered to train our base model 
 %We use 10-fold cross-validation to validate our base learner's performance, {whereby the data is divided into ten validation sets.} % This, in turn, produces...
% We improve our framework training by tuning the algorithm's hyper-parameters~\cite{scikit-learn}. Hyper-parameter tuning can provide better performance estimates for some applications. 
% {First, we perform as many iterations of the cross-validation process as hyper-parameter combinations}. %, each time using a different model setting. 
% {Second, we compare all the generated models by evaluating them on the testing set, and select the best one}. 
% The best-tuned configuration is listed in Table~\ref{tab:results} for each application. %\jgl{Do we really need to show the hyper-parameters in the table?}
% After training our RF algorithm, we can predict the time of a configurations that are \emph{not} in the training set.  Similarly, we build another model for area prediction where we use resource utilization as a \textit{label} when we train our RF algorithm.
% Choose m design points with k factors.
% Each factor divided into m equally spaced values
%  Figure  illustrates two sets of LHS samples with
% five intervals in a 2D dimension, one denoted by dots and the other
% by triangles.
\subsection{{{Target} Model Building via Transfer Learning}}
\label{subsec:ensemble_transfer}
{%the 
\namePaper provides %framework 
the ability to transfer trained \ommm{a} performance (or resource \ommm{usage}) model across different environments.}
{\namePaper~defines} a target environment $\tau_{t}$ as an environment for which we wish to build a prediction model {$\hat{f}_t$ where data collection is expensive}, and %we define 
a source environment $\tau_{s}$ as an environment %one 
 for which we can \textit{cheaply} collect many samples to build an ML model ${f}_s$. {In our case, $\tau_{s}$ is a low-cost edge FPGA-based system, while $\tau_{t}$ is a high-cost cloud FPGA-based system. } {\namePaper~then transfers the ML model for $\tau_{s}$ to $\tau_{t}$ using \ommm{an} ensemble transfer model $\hat{h}_t$.}

\head{Transfer learner} In transfer learning, a weak relationship between the base and the target environment can decrease the predictive power of the target environment model. This degradation is referred to as a \textit{negative transfer}~\cite{jamshidi2017transfer}. To avoid this, we use an ensemble %of \textit{boosting} and \textit{Bayesian probability}-based 
model trained on the transfer set (i.e., {the} \textit{few-shot learning} dataset in Figure~\ref{fig:transfer_overiew}) as our transfer learners (TLs). %We chose these specific TL methods based on our extensive empirical analysis. 
We use non-linear transfer learners because, based on our analysis ({Section}~\ref{section:relatedness_analysis}), non-linear models are able to \gs{better} capture the non-linearity present in the accelerator performance and optimization options. Our first TL is based on TrAdaBoost~\cite{dai2007boosting},  a boosting algorithm that fuses many weak learners into one strong predictor by adjusting the weights of training instances. {The motivation behind such an approach is that by fusing many weak learners, boosting can improve the overall predictions
in areas where the \ommm{individual} learners did not perform well.} We use Gaussian process regression~\cite{Gaussian} as our second TL. It is a Bayesian algorithm that calculates the probability distribution over all the appropriate functions that fit the data.  To transfer a trained model, we train both TrAdaBoost and Gaussian process regresssion, and select the best performing TL.

% For a given prediction task, individual ML-based models provide varying degrees of accuracy. This trend is common across prediction tasks and is referred to as model disagreement~\cite{xapp}. Therefore, we need an adaptive technique that selects the best performing model for each {configuration that we would like to transfer}. %We automatically detect the {strong} models and drop the weak models. 
\subsection{\namePaper Transfer Learning Algorithm}
\label{subsec:transfer_algo}
Algorithm~\ref{algo:transfer} presents \namePaper's transfer learning approach. \gs{We provide \ommm{as} input the: (1) ${f}_s$ model trained for a low-end environment, and (2) sub-sampled few-shot learning dataset \textit{c$_{tl}$}.}  %{We reuse previously built base learner ($f_s$)} by leveraging transfer learning.   Our {We use {a few} sample observations \textit{c$_{tl}$} (line~\ref{algo:tl_data}) from {both} the source and the target environments to make our transfer learners (TLs) learn how to make source environment distribution to target environment distribution.} \textit{c$_{tl}$} is a subset of c$_{doe}$. This helps us to avoid measuring all c$_{doe}$ from a cost-prohibitive target cloud environment.
\gs{We initialize the training loop to the maximum value (line~\ref{algo:tl_initial}) to run \namePaper until convergence  (line~\ref{algo:tl_initial_loop}). We normalize the input feature vector to have all the different features to be on the same scale (line~\ref{algo:tl_data}).
Using the normalized input data, \namePaper~ trains the ensemble of TLs (line~\ref{algo:tl_train}) that} transforms the performance or resource \ommm{usage} model of a source environment  $f_{s}$ to the target environment's performance or resource \ommm{usage} model $f_{t}$. %We choose the TL that has minimum transfer error . 
\ommm{We use \textit{c$_{tl}$} to generate a transfer learner $\hat{h}_t$ (line~\ref{algo:line:findTL}). We choose the TL that has the lowest mean relative error (line~\ref{algo:tl_mre}). Finally, we use $\hat{h}_t$ to transfer predictions from ${f}_s$ to produce ${f}_t$ (line~\ref{algo:tl_transform}) by performing a non-linear transformation (line~\ref{algo:tl_transfer_predict}).} %By using the  \textit{c$_{tl}$}, we generate a transfer model $\hat{h}_t$ that provides the lowest mean relative error (line~\ref{algo:tl_mre}). 
% Finally, to build ${f}_t$ from ${f}_s$ we use $\hat{h}_t$, which performs a non-linear transformation of the predictions (line~\ref{algo:tl_transform}) of ${f}_s$. 

\input{algorithms/transfer_algorithm}




%This helps us to avoid measuring all c$_{lhs}$ from a cost-prohibitive target cloud environment. 
% We select \textit{c$_{tl}$} from \textit{c$_{lhs}$} by applying {a} probability-based sampling {technique} called \textit{reservoir sampling}~\cite{vitter1985random}. %We apply a 
% {Reservoir sampling} %because it 
% assigns an equal probability of being selected to every element of %the 
% {a} population {(i.e., \textit{c$_{lhs}$})}. 
 %The intuition behind %choosing this reservoir sampling is to assign an equal probability to every element in the alreadyssampled space.
%{Using 


% To understand the notion of relatedness of the performance models in source and target environments we perform correlation analysis. The correction between the target system and the source system.


==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/relatedWork.tex <==
\section{Related Work}
% \vspace{-0.1cm}
To our knowledge,  {\namePaper} is the first work to {leverage an ML-based performance and resource {usage} model trained for a low-end \om{edge environment} to predict \ommm{the} performance and resource {usage} of an accelerator implementation for a new, high-end cloud environment.}  FPGAs  {lead to} very low productivity due to the time-consuming downstream accelerator implementation process. %We have extensively evaluated our approach using five FPGA-based platforms with three different interconnect technologies on six real-world applications. 
In this section, we describe other related works in ML-based modeling \ommm{of FPGA}, analytical  modeling \ommm{of FPGA}, and transfer learning.

\noindent\textbf{ML-based modeling  \ommm{of FPGAs}.} Recent works propose ML-based methods~\cite{makrani2019pyramid,ferianc2020improving,ustun2020accurate,o2018hlspredict,xppe_asp_dac,dai2018fast,zhao2019machine,yanghua2016improving,wang2020machine,mahapatra2014machine,sun2022correlated} to overcome the issue of low productivity while designing FPGA-based accelerators. O'Neal~\etal~\cite{o2018hlspredict} use CPU performance counters to train several ML-based models to predict \omu{the} performance and power consumption of an accelerator implementation. Makrani~\etal~\cite{xppe_asp_dac} train a neural network-based model to predict application speedup across different FPGAs. Makrani~\etal~\cite{makrani2019pyramid} and Dai~\etal~\cite{dai2018fast} use ML to predict resource \ommm{usage} for an accelerator implementation. %post-implementation resource utilization from pre-implementation results. 
However, these solutions become largely impractical once the platform, the application, or even the size of the workload changes. \namePaper~proposes to reuse previously\ommm{-}built models for a low-end source environment on a high-end target environment through transfer learning. Unlike \namePaper, past works apply traditional, time-consuming brute-force techniques to collect\omu{s} training datasets. %These techniques quickly become intractable when the number of optimization parameters increases due to the curse of dimensionality~\cite{bellman1966dynamic}.
% Moreover, FPGAs are deployed with a host system, and often past works ignore the overhead of data transfer between the host and the FPGA, which makes their model incompetent for the heterogeneous systems. In our work, we consider end-to-end system performance and leverage transfer learning to build models for different platforms and different applications. 
% Moreover, past works~\cite{tulikaML} apply traditional, time-consuming brute-force techniques to collect training dataset. These techniques quickly become intractable when the number of optimization parameters increases due to the curse of dimensionality~\cite{bellman1966dynamic}. 
% In this work, we leverage \textit{design of experiment} techniques to reduce the training overhead dramatically and still build accurate models. 

\noindent\textbf{Analytical modeling  \ommm{of FPGAs}.} {Analytic\ommm{al} models abstract low-level system details and
provide quick performance estimates at the cost of accuracy. These approaches \ommm{(e.g.,}~\cite{linAnalyzer,zhao2017comba,hlsscope,chai_icpe19}) analyze dataflow graphs and apply mathematical equations to approximate resource usage or performance after the HLS pre-implementation phase. \ommm{Even though they} enable {quick early-stage design studies, however, analytical models} are not able to model the intricacies of the complete  implementation process~\cite{dai2018fast}. Therefore, these approaches provide crude estimates of the actual performance. Moreover, these models require \ommm{FPGA domain} knowledge to form mathematical equations.  In contrast,~\namePaper~does not require expert knowledge to construct equations. \namePaper~learns from the \ommm{training} data \ommm{(application features and accelerator optimization options) to consider} the complete downstream accelerator implementation process and provides the capability to transfer models from an edge-FPGA to a high-end cloud FPGA environment.}

%  LEAPER is the first method to deal with transfer learning on FPGAs, which are infamous for low productivity due to the time-consuming downstream implementation process. \namePaper~not only performs configuration prediction (Figure~\ref{fig:transfer_overiew} ``Base model building'' stage) but also provides the ability to transfer the models (Figure~\ref{fig:transfer_overiew} ``Target model building - Few-shot learning'' stage). \namePaper~is orthogonal to previous approaches (ML and non-ML) as it also provides the ability to ``transfer'' models in milli-seconds (\textit{ref}. Table~\ref{tab:timing}).   Additionally in this work, we leverage \textit{design of experiment} techniques to reduce the training overhead dramatically and still build accurate models. 
 %We believe LEAPER can open up new avenues for research on the cloud FPGA-based systems 


% Some works have proposed the use of white-box model techniques for quick performance prediction. However, these techniques have two main limitations. First, it relies on analytical or design models derived from mathematical
% theories or software architecture abstraction, which are often imprecise~\cite{chen2016generating}. Second, coarse analytical models abstract detailed phenomena  that influence the overall application behaviour.
% Our approach  is orthogonal to these approaches and proposes a new way to EDA by reusing previously built model on cheaper sources to accelerate the learning of models on other target platform or applications through transfer learning.





% For a given data parallel application, achieving the best performance on a hetergogneous platform not oonly depends on the performance xplpoitation of eath single processing unit, but also on the perfromance aggregarion of the entire system. That is to say progrormmers have to partition the applicaiton workload such that all the processing units are best utilized and combined to achieve the best aggregate performance.  fingind such a wokrload paritioning remains a challenge~\cite{shen2015workload}. First, the heterogeneity of the platform requires the partitioning ot fully consider the the processing units' difference in processing capabiliyt, hardware archiecture, memory model, external bus. Secondly, the diversity of platforms, applicaitons, and datasets increases the partitioning complexity. Finally, from the programmer's viewpoint, it is challenging to obtain with limited time and effort the optimal partitioning that leads to the best performance for a given heterogenous platform, application, and dataset.


\noindent\textbf{Transfer learning.} Recently, transfer learning~\cite{chen2010experience,pan2009survey,baumann2018classifying,bozinovski1976influence,pratt1992discriminability} has gained traction to decrease the cost of learning by transferring knowledge \ommm{between different tasks}. % and can overcome {concept drift}~\cite{concept_drift}.  
Valov~\etal~\cite{valov2017transferring} investigate the transfer of application models across different CPU-based environments using linear transformations. Jamshidi~\etal~\cite{jamshidi2017transfer} demonstrate the applicability of using nonlinear models to transfer CPU-based  performance models. {The works above influenced the design of~\namePaper}. In contrast \ommm{to them}, we:  (1) focus on FPGA-based systems that, unlike a CPU-based system, ha\ommm{ve} a different hardware architecture for every application and optimization strategy, and % is not static and changes with an application or optimization strategy, and (2) tailor the hardware circuitry to an application by leveraging the large high-dimensional optimization space and has very low productivity due to the time-consuming downstream implementation process. Moreover, we 
(2) use an ensemble of transfer learners that transfers accurate models to a target environment. \\

==> LEAPER_ICCD'22_Camera_ready_FINAL/sections/results.tex <==
%\section{Evaluation and Results}
\section{{Evaluation \gs{Methodology}}}
\label{sec:evaluation}




\subsection{Hardware Platform}
\label{subsec:eval_platform}
% With a high adoption of FPGAs in the cloud, various emerging CPU-FPGA platforms with competing cache-coherent interconnect standards are being developed, such as  %high-bandwidth} 
%  the IBM Coherent Accelerator Processor Interface (CAPI)~\cite{openCAPI}, the Cache Coherent Interconnect for Accelerators
% (CCIX)~\cite{benton2017ccix}, the Ultra Path Interconnect (UPI)~\cite{UPI} and the Compute Express Link (CXL)~\cite{sharma2019compute}.  

% {The benefits of employing such cache-coherent interconnect links for attaching FPGAs to CPUs, as opposed to the traditional DMA-like communication protocols (e.g. PCIe), are not only the ultra lower-latency and the higher bandwidth of the communication, but most importantly, the ability of the accelerator to access coherently the entire memory space of the CPU, without consuming excessive CPU cycles. Traditionally, the host processor has a shared memory space across its cores with coherent caches. Attached devices such as FPGAs, GPUs, network and storage controllers are memory-mapped and use a DMA to transfer data between local and system memory across an interconnect such as PCIe. Attached devices can not see the entire system memory, but only a part of it. Communication between the host processor and attached devices requires an inefficient software stack, including user-space software, drivers and kernel-space modules, in comparison to the communication scheme between CPU cores using shared memory. Especially when DRAM memory bandwidth becomes a constraint, requiring extra memory-to-memory copies to move data from one address space to another is cumbersome~\cite{Fang2020}. This is the driving force of the industry to push for coherency and shared memory across CPU cores and attached devices, like FPGAs. This way, the accelerators act as peers to the processor cores. %For example, one of the earliest industry-adopted paradigms of cache coherency for accelerators was the Cell Broadband Engine architecture~\cite{5388817}, which introduced coherent shared system memory access for its Synergistic Processor Element accelerators.

% Based on this upcoming trend, in this work we adopt cache-coherent FPGA accelerators, both for the low-end and the high-end systems. Specifically, 
Table~\ref{tab:systemparameters} summarizes the system details of our low-end edge environment and {high-end cloud} environment. We select \ommm{the} widely available PYNQ-Z1 board~\cite{pynq} with XC7Z020-1CLG400C FPGA~\cite{zynq} as the low-end FPGA platform to build base model. We use the accelerator coherency port (ACP)~\cite{ACP} with PCIe Gen2  \ommm{to} attach FPGA-based accelerators to the ARM Cortex-A9 CPU~\cite{cortexA9} present \ommm{in} PYNQ-Z1. %The XC7Z020 FPGA on PYNQ-Z1 is connected to ARM Cortex A9 CPU via PCIe Gen2 interconnect.  
We use \ommm{the} Nimbix cloud~\cite{nimbix} with CAPI-based FPGA system attached to a server-grade IBM POWER9 CPU system as our high-end cloud environment. \ommm{Nimbix} uses KVM (Kernel Virtual Machine)~\cite{kvm} for Linux virtualization and OpenStack~\cite{openstack} as  middleware. We evaluate five state-of-the-art, high-end, cloud FPGA boards (ADM8K5~\cite{ad8k5}, ADM9V3~\cite{ad9v3}, NSA241~\cite{nsa241}, N250SP~\cite{250SP}, and ADMKU3~\cite{adku3}) using two different interconnect technologies (CAPI-1 and CAPI-2). We can derive from the indicative prices listed in the last column of  Table~\ref{tab:systemparameters} \ommm{shows} that the  total cost of ownership (TCO) of a high-end cloud system can be more than $100\times$ of that of the low-end system, and thus it can be cost-prohibitive %for a bare-metal deployment 
to many users.%In addition, we select a Coherent Accelerator Processor Interface (CAPI)~\cite{stuecheli2015capi}-based system as the target platform because it provides the most matured coherent accelerator-based ecosystem with a production-ready cloud offering through Nimbix Cloud~\cite{nimbix}.
 %Complementary, moving a workload to a cloud FPGA instance should offer such a speedup that it compensates for the extra design time, effort, and cost of this decision by the end-user. \namePaper helps a user to rapidly quantify such a decision by experimenting with low-cost and broadly available FPGAs, like the PYNQ-Z1.




\input{tables/hardware.tex}


\subsection{Programming Toolflow}
% For accelerator implementation and deployment, we leverage CAPI-compatible tools offered by Xilinx. 

We use the {Xilinx} SDSoC~\cite{sdsoc} design tool for implementing an accelerator on the low-end edge environment
$\tau_{s}$ and the Vivado HLS~\cite{hls} with \ommm{the} IBM CAPI-SNAP framework\footnote{https://github.com/open-power/snap} for the high-end cloud environment $\tau_{t}$. The SNAP framework provides seamless integration of an accelerator~\cite{10.1007/978-3-030-34356-9_25} and allows \ommm{the} exchange of control signals between the host and the FPGA processing elements over the
AXI lite interface~\cite{axilite}. 

% On the cloud system, we use KVM image with FPGA and SoC development tools, IPs, and licences to generate bitstreams for the selected Xilinx devices in Table~\ref{tab:systemparameters}. 

%, model, which is transferred to different platforms/applications using our ensemble transfer learners.

 

% \begin{SCfigure}[][h]
% \vspace{1.2cm}
% \centering
%     \resizebox{0.35\textwidth}{!}{
%      \includegraphics[width=0.65\linewidth,trim={0.4cm 0.3cm 0.7cm 0.1cm},clip]{images/System.pdf}
% }
% \caption{CAPI-based platform with IBM\textsuperscript{\textregistered} POWER9 used for target model.
% \label{fig:system}}
% \vspace{-1.4cm}
% \end{SCfigure}

%  \begin{figure}[t]
%  \vspace{-0.4cm}
% \centering
% \begin{subfigure}[t]{.28\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/System.pdf}
%   \vspace{-0.5cm}
%   \caption{
%   \label{fig:system}}
% \end{subfigure}%
% \begin{subfigure}[t]{.22\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/Execution_timeline_5.pdf}
%   \vspace{-0.5cm}
%   \caption{
%   \label{fig:execution}}
% \end{subfigure}
%  \vspace{-0.2cm}
% \caption[Two numerical solutions]{(a) CAPI-based accelerator platform with IBM\textsuperscript{\textregistered} POWER9 (target platform). FPGA acts as a peer to the CPU by accessing the main memory through a high-performance cache-coherent CAPI link, enabled by PSL. (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard FPGA memory. A software-defined API handles %offloading jobs 
% {job-offloading} to accelerators with an interrupt-based queuing mechanism that allows minimal CPU consumption (power) during FPGA use. \label{fig:system}}
 
% % \vspace{-1cm}
%  \vspace{-0.4cm}
% \end{figure}

% \subsection{Target Platform Accelerator Generation}
% \vspace{-0.05cm}
% The CAPI SNAP framework is an open-source environment that establishes two technology novelties~\cite{wenzel2018getting}: (1) it enables application programmers to embrace FPGA acceleration and CAPI's technology benefits, and (2) it places the accelerated compute engines, or \textit{actions}, closer to the data to achieve better performance. SNAP provides a simple API to call for an accelerated \textit{action}, and also provides programming methods to code customized accelerated \textit{actions} on the FPGA side. These accelerated \textit{actions} can be specified in C/C++ code, which is then compiled to the FPGA target using the Xilinx Vivado HLS tool. 
% \jgl{This entire paragraph is about the evaluation setup. This should go into Evaluation Methodology. Your work is more general than IBM CAPI. You could use it on other systems. CAPI systems are just the evaluation setup. {but we have acceleration generation as well, how could we describe that?}}

%  \begin{figure*}[t]
%  % \hspace{0.9cm}
%   \begin{subfigure}{0.495\textwidth}
%   %\vspace{-0.1cm} 
%   \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/across-board-blstm2.pdf}
%   %  \vspace{-0.8cm}
%     %  \caption{}
%     \label{fig:board_blstm}
%   \end{subfigure}
%   \begin{subfigure}{0.495\textwidth}
%   %\hspace{-0.1cm}  
%   \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/across-board-cedd2.pdf}
%   %  \vspace{-0.3cm}
%   % \caption{ \hspace*{1.5cm}}
%   % \caption{}
%     \label{fig:board_cedd}
%   \end{subfigure}
%   \begin{subfigure}{0.495\textwidth}
% %\hspace*{0.9cm}
% \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/across-board-digit2.pdf}    %\vspace{-0.8cm}
%   % \caption{\hspace*{-1.8cm}}
%     %\caption{}
%     \label{fig:board_digit}
%   \end{subfigure}
%   %\hspace{1.1cm}
%   \begin{subfigure}{0.495\textwidth}
%     \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/across-board-hist2.pdf}
%   % \vspace{-0.8cm}
%     %\caption{}
%     \label{fig:board_hist}
%   \end{subfigure}
%      \begin{subfigure}{0.495\textwidth}
%     \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/across-board-sc2.pdf}
%   % \vspace{-0.8cm}
%     %\caption{}
%     \label{fig:board_sc}
%   \end{subfigure}
%      \begin{subfigure}{0.495\textwidth}
%     \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{imagescr_ac.pdf}
%   % \vspace{-0.8cm}
%     %\caption{}
%     \label{fig:board_select}
%   \end{subfigure}
%     \vspace{-0.3cm}
%   \caption{\namePaper's accuracy for %transferred
%   {transferring} base models across CAPI-enabled {cloud} FPGA-based systems. {The legends indicate the target platforms}. The base model was trained on a low-end PYNQ-Z1 board and, for each application, we \textit{transfer} this model to different high-end cloud FPGA-based %HPC 
%   platforms using different samples {(horizontal axis)} from the target platform. }%Once trained using \textit{few shot}, the transferred model makes predictions for all other configurations in the target platform.} % \jgl{Why don't we show results for 0 samples? That would show how effective the transfer learning is.}}
%   \label{fig:acros_board}
% %   \vspace{-0.5cm}
% \end{figure*}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{images/cr_across-board2.pdf}
  \vspace{-15pt}
  \caption{\namePaper's accuracy for %transferred
%   {transferring} base models across CAPI-enabled {cloud} FPGA-based systems. {The legends indicate the target platforms}. The base model was trained on a low-end PYNQ-Z1 board and, for each application, we \textit{transfer} this model to different high-end cloud FPGA-based %HPC 
  platforms using different samples {(horizontal axis)} from the target platform. }%Once trained using \textit{few shot}, the transferred model makes predictions for all other configurations in the target platform.} % \jgl{Why don't we show results for 0 samples? That would show how effective the transfer learning is.}}
  \label{fig:acros_board}
%   \vspace{12pt}
\end{figure*}

 \begin{figure*}[t]
 % \hspace{0.9cm}
  \begin{subfigure}{0.495\textwidth}
   %\vspace{-0.1cm} 
   \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_blstm_cr1.pdf}
     \vspace{-0.3cm}
    %  \caption{}
    \label{fig:app_blstm}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
  %\hspace{-0.1cm}  
  \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_cedd_cr1.pdf}
    \vspace{-0.3cm}
   % \caption{ \hspace*{1.5cm}}
   % \caption{}
    \label{fig:app_cedd}
  \end{subfigure}
   \begin{subfigure}{0.495\textwidth}
%\hspace*{0.9cm}
\includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_digit_cr1.pdf}    \vspace{-0.3cm}
   % \caption{\hspace*{-1.8cm}}
    %\caption{}
    \label{fig:app_digit}
    %\vspace{-1.5cm}
  \end{subfigure}
  %\hspace{1.1cm}
   \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_hist_cr1.pdf}
   \vspace{-0.3cm}
    %\caption{}
    \label{fig:app_hist}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_se_cr1.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:app_sc}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
  %   \includegraphics[width=\textwidth,trim={2.7cm 10cm 2cm 10cm},clip]{images/gagan_across-app-select.pdf}
     \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{images/app_select_cr1.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:app_select}
  \end{subfigure}
\vspace{-14pt}
  \caption{\namePaper's accuracy for %transferred 
  {transferring} base models across various applications. {The legends indicate the number of samples}. Each plot represents a different application \ommm{used as a base model}. We \textit{transfer} these base models, trained on the PYNQ-Z1 platform. %, by using invariant configuration features to build a target application model. 
  } %\jgl{Why don't we show results for 0 samples? That would show how effective the transfer learning is.}}
   \label{fig:across_app}
    %  \vspace{-0.5cm}
\end{figure*}

% We aim to minimize the prediction error and the model training cost under FPGA area constraint. So it is a multi objective optimization problem
%We consider different

\subsection{Workloads} 
\label{subsec:eval_workload}
We evaluate \namePaper~using six
 benchmarks (Table~\ref{tab:app_details}), which are hand-tuned for FPGA execution. %, that 
These benchmarks cover %a wide range of 
{several application} domains, i.e., \textbf{(1) image processing}:  histogram {calculation (\textit{hist})~\cite{gomezluna2017chai}, and canny edge detection (\textit{cedd})~\cite{gomezluna2017chai}}; \textbf{(2) machine learning}: binary long short term memory (\textit{blstm})~\cite{diamantopoulos2018ectalk}, digit recognition (\textit{digit})~\cite{zhou2018rosetta}; %and canny edge detection (\textit{cedd})~\cite{gomez2017chai}; 
%and 
\textbf{(3) databases}: relational operation (\textit{select})~\cite{gomezluna2015ds}; 
and \textbf{(4) {data reorganization}}: stream compaction (\textit{sc})~\cite{gomezluna2017chai}. These kernels are specified in C/C++ code using high-level synthesis (HLS) that is compiled to the target FPGA device.

\input{tables/application}
% %LHS is applied to these workloads to select a small set of optimizations $c_{lhs}$ that represent the entire space of possible optimizations. Next, we implement and deploy %the
% FPGA accelerators using {Xilinx} SDSoC for %the
% $\tau_{s}$ and Vivado HLS with IBM CAPI-SNAP framework\footnote{https://github.com/open-power/snap} for $\tau_{t}$. Finally, we train our base learner and leverage it to {perform predictions for a new, unseen cloud target environment}. 

\subsection{Evaluation Metrics}
\label{subsec:eval_metric}
\namePaper~is used to transfer a trained model using \textit{few-shot learning}. We then analyze the accuracy of the newly-built target model to predict the performance and resource \ommm{usage} of all the other configurations in %the 
\ommm{the target environment}. %optimization space.
We evaluate the accuracy of the %the proposed 
{transferred} model in terms of the mean relative error ($\epsilon_i$) to indicate the proximity of the predicted value $y_{i}^\prime$ to the actual value $y_{i}$ across \textit{N} test samples. The mean relative error (MRE) is calculated with Equation~\ref{eq:2}.
% \vspace{-0.08cm}
\begin{align}
 MRE= \frac{1}{N} \displaystyle \sum_{i=1}^{N} \epsilon_i=\frac{1}{N} \displaystyle \sum_{i=1}^{N}\frac{|y_{i}^\prime -y_{i}|}{y_{i}}    
\label{eq:2}
\end{align}
% \vspace{-0.05cm}

\section{\gs{Results}}
\label{sec:result}
% \subsection*{Transfer Across Platforms and Applications}
\subsection{Accuracy Analysis \ommm{of the} Transferred Model}
\noindent {\textbf{Performance model transfer.}}
Figure~\ref{fig:acros_board} shows \namePaper's accuracy for transferring \omu{from edge to {cloud} platforms}. We make the following three observations. First, as we increase the number of labeled samples, the target model accuracy increases. However, the accuracy saturates and  with 5-10 \gs{samples} or \textit{shots}, we can achieve an accuracy as high as 80-90\%. Second, compared to applications with multiple complex kernels (\textit{blstm}, \textit{cedd}, \textit{digit} \omu{in Figure~\ref{fig:acros_board}(a), \ref{fig:acros_board}(b), and \ref{fig:acros_board}(c), respectively)}, simpler kernels (\textit{hist}, \textit{sc}, \textit{select} \omu{in Figure~\ref{fig:acros_board}(d), \ref{fig:acros_board}(e), and \ref{fig:acros_board}(f), respectively)} can be {more} easily transferred using fewer samples. \gs{There are two reasons for this trend: (1)} applications with multiple kernels have a larger optimization space. The large optimization space leads to more complex interactions that have compounding effects with other optimization options because we  %trying to optimize 
\ommm{model} multiple kernels rather than just a single~kernel, and
(2) simple kernels such as \textit{sc} and \textit{select} have been implemented using \textit{hls stream} interfaces, where rather than storing intermediate data in local FPGA memories, we read streams of data, and hence certain complex optimizations (like array partitioning) cannot be applied. This leads to a change in the feature space for different environments.
%\jgl{I don't see how this sentence is relevant for the observations}.  
%Third, %change 
 %change in the technology node from one FPGA to another (e.g., changing from ADMKU3 board to  AD9V3 board) has a lower impact than changing the external bandwidth to a new interconnect standard on the {transferring} process.
Third, \ommm{similar environments} are more amenable to transfer as the source, and target models are more closely related, \omu{i.e., we require small number of samples from the target environment to transfer a model. For example,} %change 
{transferring} to an FPGA with CAPI1 interface {(PCIe Gen3 with $\sim$~3.3 GB/s bandwidth)} %is 
from low-end PYNQ with PCIe Gen2 $\sim$~1.2 GB/s bandwidth entails a smaller \ommm{increase} in bandwidth %technology 
than moving to an FPGA with CAPI2 interface {(PCIe Gen4 with $\sim$~12.3 GB/s bandwidth)}. 

Figure~\ref{fig:across_app} shows \namePaper's accuracy for transferring ML models \emph{across different applications}. \gs{We make three observations.}
First, as we increase the number of training samples, the target model accuracy increases for most of the applications. \gs{This observation is inline with the observation we made while transferring models performance models across different cloud platforms (Figure~\ref{fig:acros_board}).}
Second, the \ommm{largest}  improvement %happened
{in accuracy occurs} when our sample size $(c_{tl})$ %was
{is} between 2 to 10. In most cases, {the accuracy} saturates after 20 samples. 
{Third}, in some cases, we see a decrease in accuracy {when increasing the number of samples}, e.g., Figure~\ref{fig:across_app}(a) for \texttt{HIST}, \texttt{SC}, and \texttt{SELECT}. This result could be attributed to training with a small amount of data, which can sometimes lead to overfitting~\cite{dai2007boosting}. 
%Further, in 
\gs{We conclude that \namePaper is \ommm{effective at} transferring models \omu{from edge to} cloud platforms and \ommm{across} applications.}
% In Section~\ref{section:relatedness_analysis}, we %provide explainability of 
% {further explain} our results by measuring the divergence of performance distributions to quantify the statistical distance between the source and target models. 
\\


\noindent \textbf{Resource \ommm{usage} model transfer.} By using \namePaper, %~approach, 
we can also train a resource \ommm{usage} model on a \textit{low-end} edge environment and transfer it to a high-end cloud environment.  Figure~\ref{fig:area_transfer} shows the accuracy of a target model trained by \textit{5-shot} {transfer} learning for predicting %configuration 
{a} resource \ommm{usage} vector $\eta_{\{BRAM, FF, LUT, DSP\}}$. The reported accuracy is for the transferred model, i.e., using a base model (low-end FPGA) to predict a target model (high-end cloud FPGA) after \gs{transfer} learning. In Figure~\ref{fig:area_transfer}(a), the horizontal axis depicts the target platform, while the base model is trained on a PYNQ-Z1 board. In the case of \ommm{across application} transfer (Figure~\ref{fig:area_transfer}(b)), the platform remains unchanged (PYNQ-Z1),  \ommm{while we use different applications to build the base model (horizontal axis).}

We make %two 
three observations. First, the resource \ommm{usage} model shows low error rates for predicting BRAM and DSP \ommm{usage}. This is attributed to the fact that the technological configuration of these resources remains relatively unchanged across platforms (e.g., BRAM is implemented as 18 Kbits in both the source and target platforms). Second, flip-flops and look-up-tables have %a 
comparably \ommm{lower accuracy} %that is
because the configuration of CLB slices varies with %change in 
{the} transistor technology and FPGA family. {Third, while transferring across different applications (Figure~\ref{fig:area_transfer}(b)), we observe} relatively low accuracy for DSP \ommm{usage} while transferring a base model trained on \textit{hist}. This low accuracy is because the \textit{hist} accelerator implementation do\ommm{es} not use DSP units for logic. However, all other applications \ommm{use} DSP \ommm{units}. Therefore, the ML model trained on \textit{hist} \ommm{provides lower accuracy} in other environments \ommm{that use DSP units for accelerator implementation}. \gs{We conclude that \namePaper can efficiently transfer resource \ommm{usage} models.} %Figure~\ref{fig:area_app} shows the mean accuracy for transferring different application-based models on a fixed FPGA board. %In this figure, we see a

\begin{figure}[h]
\begin{subfigure}[b]{\linewidth}
\centering
   %\includegraphics[width=1\linewidth,trim={2.2cm 8cm 0cm 7cm},clip]{images/area_board.pdf}
   \includegraphics[width=\linewidth]{images/area-board-2.pdf}
         \phantomcaption
    \label{fig:area_board} 
    % \vspace{0.1cm}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
\centering
   %\includegraphics[width=1\linewidth,trim={1.8cm 12cm 0.5cm 12cm},clip]{images/area_app.pdf}
   \includegraphics[width=\linewidth]{images/area-app-2.pdf}
      \phantomcaption
    \label{fig:area_app}
%   \caption{\label{fig:area_app}}

\end{subfigure}
\vspace{-0.9cm}
\caption[Two numerical solutions]{\namePaper's accuracy for transferring FPGA resource usage models through using (a) a base \ommm{model} trained on a low-end PYNQ-Z1 to different high-end target FPGA boards (horizontal axis), and  (b) different applications as base \ommm{models} (horizontal axis) to all the target applications, on low-end PYNQ-Z1 board.
% \gaganCheck{Could we change x-axix from target model to target FPGA/platform}
}
\label{fig:area_transfer} 
\end{figure}
\vspace{0.2cm}

In Table~\ref{tab:low_high_end}, we \ommm{report} the performance and resource \ommm{usage} for our \ommm{six} applications both on a low-end system and a high-end ADMKU3 FPGA-based cloud system. We use \namePaper to obtain the performance and resource \ommm{usage} for the high-end cloud configuration.
\input{tables/values}




\subsection{Base Model Accuracy Analysis}
We also evaluate the accuracy of our base model. The base model is trained on our low-end edge PYNQ board using $c_{lhs}$ configurations sampled using \ommm{the} DoE technique. The base model can predict performance (or resource \ommm{usage}) outside the base model dataset (i.e, any configuration that is not a part of the DoE configuration space) $c_{lhs}$. To assess our base model, we use 30 previously unseen configurations that are not part of $c_{lhs}$ on the base system, and we evaluate the mean relative error for all 30 unseen configurations on all six applications.  Figure~\ref{fig:base_mode} shows the base model accuracy results. We also compare our base model to three other ML algorithms
that are also trained using $c_{lhs}$ configurations to predict performance and resource \ommm{usage}: XG-Boost (\texttt{XGB})~\cite{chen2016xgboost} based on  Dai~\etal~\cite{dai2018fast},
an artificial neural network (\texttt{ANN}) used by Makrani~\etal~\cite{xppe_asp_dac} and a traditional
decision tree (\texttt{DT})~\cite{loh2011classification}. 

 \begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.1cm 0.1cm 0.1cm},clip]{images/BASE_MODEL_FPGAS.pdf}
  \vspace{-14pt}
  \caption{\ommm{Average} accuracy for performance (\texttt{Exec.}  \texttt{Time}) and resource  (\texttt{BRAM}, \texttt{DSP}, \texttt{FF}, \texttt{LUT}) \ommm{usage} predictions using \namePaper's base model and other machine learning techniques.}
  \label{fig:base_mode}
  %\vspace{-0.5cm}
 \end{figure}
 \vspace{0.2cm}
We make two major observations. First, on average, \namePaper~is \gss{8.1\% (4.1\%),	4.3\% (5.1\%), and	25.9\% (23.9\%) more accurate in terms of performance (resource \ommm{usage}) prediction than \texttt{XGB}, \texttt{ANN}, and \texttt{DT}, respectively. %Second, \texttt{XGB}  provides 4.1\% lower accuracy than \texttt{ANN} for performance prediction while  1.2\% higher accuracy for resource \ommm{usage} prediction. When compared to \texttt{DT},  \texttt{XGB} provides 19.5\%  (20.6\%) higher accuracy for performance (resource \ommm{usage}) prediction. Third, 
Second, \texttt{ANN} is  22.7\% and 19.5\% more accurate than  \textit{DT} for performance and resource \ommm{usage} prediction, respectively, but performs \ommm{worse}
than \namePaper. \texttt{ANN} is not sample-efficient as it requires more training samples to learn~\cite{li2018processor}.}  \gs{We conclude that \namePaper's base model provides both high accuracy and sample-efficiency compared to other ML-based algorithms.}

We also compare the performance of using different \ommm{ML-based methods} for transferring models across different platforms and across different applications.
In Table~\ref{tab:compare}, we show the average accuracy of \namePaper's ensemble of transfer learner and compare it to two different \ommm{ML-based methods}: (1) decision tree (\texttt{DT})~\cite{loh2011classification}, and (2) adaBoost (\texttt{ADA})~\cite{adaboost}. %We observe that our ensemble of TLs are able to outperform both \texttt{DT} and \texttt{ADA}. 
We observe that \namePaper is \ommm{on average} 12.1\% (10.6\%) and 6.6\% (7.7\%)  on average more accurate in transferring models across platforms (across applications) than \texttt{DT} and \texttt{ADA}, respectively. We conclude that an ensemble of \ommm{transfer learner} is better than using a single \ommm{transfer learner} while transferring across different FPGA-based environments.
 
\input{tables/compare.tex}


\subsection{Target {Cloud FPGA }Model Building Cost}
\label{subsection:timing}
\gs{In Table~\ref{tab:timing}, we mention the time and cost to build a model from scratch on a cloud environment using the traditional \ommm{ML-based} approach and compare it to using \namePaper to build a model for the cloud environment.}
If we build a model from scratch, then we need 50 sampled DoE configurations ($c_{lhs}$) for which the time and cost is mentioned in \textit{DoE run %(mins)
(hours)} and \textit{DoE cost}, respectively. Table~\ref{tab:timing} also includes the {execution} time %for execution 
on the ADMKU3 {cloud} platform (``Exec (msec)''. While the process of synthesis and place and route (P\&R) for the cloud FPGA, which is needed to obtain performance estimates in terms of maximum operating clock frequency and the resource \ommm{usage}, can be carried out offline, most of the cloud providers offer virtual machines (VMs) with all the appropriate software, IPs, and licenses needed to generate an FPGA image ready to be deployed at their cloud infrastructure (e.g., the Vivado AMI of AWS~\cite{AMI}). Therefore, we include the cost of the cloud environment (``Est. Cost (\$)'') for data collection.



By using \namePaper, the DoE runtime is amortized and, by using a few labeled samples $c_{tl}$ (``5-shot (hours)'') from the target platform, we can transfer a previously trained model and make predictions for all the other configurations for the target platform. We mention the the transfer time (``Transfer (msec)'') for each model. 
{As a result}, quick exploration and {significant} time savings {(at least 10.2$\times$) are possible when transferring a model (i.e., ``5-shot (hours)'' + ``Transfer (msec)'') as compared to building a new model from scratch (i.e., ``DoE run (hours)'') + ``Exec (msec)'')}. DoE reduces training samples from 500+ to 50, while  \textit{5-shot} transfer learning further reduces the number of samples to 5, so we achieve $\sim100\times$ effective speedup compared to a traditional ``brute-force'' approach for data collection.

\input{tables/timing.tex}






\section{\gs{Explainability: Why does \namePaper~work?}}
 \label{section:relatedness_analysis}
{To explain our results for transfer learning}, we analyze the degree of \textit{relatedness} between the source and target environments. 
We use two different analysis techniques: (1) divergence analysis~\cite{coutinho2011divergence}, and (2) correlation analysis~\cite{benesty2009pearson}.

\head{Divergence analysis} We use Jensen-Shannon divergence (JSD)~\cite{jsd} to measure  the difference between two probability distributions of the source ($P(\tau_{s})$) and the target environment ($P(\tau_{t})$). %We measure the relatedness of the performance distributions of the source ($P(\tau_{s})$) and the target applications  ($P(\tau_{t})$). This analysis measures the degree of non-linearity.
% We use this analysis only to analyze transfer between applications on the same platform because application-based environments exhibit a low linear correlation.
% because application-based environments exhibit a low linear correlation. 
%We use the Jensen-Shannon Divergence (JSD)~\cite{jsd} (Table~\ref{tab:jsd}) to quantify the statistical distance between $P(\tau_{s})$ and $P(\tau_{t})$. 
The lower the JSD \ommm{value}, the more similar the target environment is to the source (i.e., if $D_{JSD}(P(\tau_{t}) || P(\tau_{s})=0$ implies that the distributions are identical and 1 indicates unrelated distributions). Table~\ref{tab:jsd} shows the JSD analysis for transferring models between different applications. We make three main observations. First, JSD analysis confirms the trend observed from transferring application models (Figure~\ref{fig:across_app}), i.e., the more closely related the source and target applications, %are 
the fewer %numbers of 
samples are required to train our non-linear transfer learners. Second, the higher the JSD between two applications, the lower the accuracy while transferring between those tasks. %the measured JSD between the tasks is proportional to the error of the target task. 
Third, for many applications JSD values is low, which indicates that we can easily transfer models between such environments using a few samples from the target environment. %Similar trends are observed for the resource utilization model.


\input{tables/jsd.tex}


\head{Correlation analysis} \ommm{Correlation analysis} measures the strength of linear correlation between two environments. We make four major observations. First, for different target hardware platforms, we have a high correlation of $0.76$ to $0.97$ {between the source and target  execution time}, which indicates that the target model's performance behavior can \ommm{accurately} be learned using the source environment.  
%
Second, as we switch to a higher external bandwidth {for the target platform (i.e., CAPI1 to CAPI2)}, 
the correlation becomes lower because the hardware change is much more \textit{severe} coming from a low-end FPGA with limited external bandwidth.  \omu{Whereas changing the technology node from one FPGA to another (e.g., changing from ADMKU3 board to  AD9V3 board) leads to a smaller change in the environment because of the linear relation between technology node and performance. }
%  \ommm{Third, \omu{transferring models from PYNQ-Z1 to cloud} change in the external bandwidth to a new interconnect standard leads to a bigger change in environment than changing the technology node from one FPGA to another (e.g., changing from ADMKU3 board to  AD9V3 board). } 
%Third, compared to using a single transfer learner, an ensemble of learners %was 
%can perform more accurate and robust predictions (\textit{ref.} Figure~\ref{fig:acros_board}, \ref{fig:across_app}, and~\ref{fig:area_transfer}). 
Third, the correlation between applications on a single platform is lower ($0.45$ to $0.9$) because of {the} varying application characteristics {and optimization space.} Fourth, as the linear correlation is not 1 for all platforms, the use of a nonlinear transfer models is substantiated. We conclude that \namePaper learns differences in environments to accurately transfer FPGA-based system  performance prediction models \omu{from one platform to another.}

% \todo[inline]{add performance numbers}
% \todo[inline]{cost on the cloud}
% ig{
% \subsection{\textbf{Use Case 1:} FPGA Suitability Analysis}
% In this section, we use \namePaper to perform an FPGA-suitability analysis, i.e., to assess the potential benefit of offloading a workload to an FPGA. 
% This analysis compares the performance of executing a workload on an FPGA, which we obtain from \namePaper's predicted FPGA performance, to the {measured performance} of executing the workload on a CPU.

% In order to obtain performance results for the host system, we use a POWER9 system with 16 cores each supporting four-thread simultaneous multi-threading. 
% \subsection{\textbf{Use Case 2:} Cost Optimization}


% }


==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/application.tex <==
\vspace{0.25cm}
\begin{table}[h]
  \caption{\gagan{Evaluated application description including their domain, major kernels, and the input dataset. For major kernels, we mention the optimization space where $\times$ represents the optimization being applied to multiple loops or elements. %\ommm{see} Table~\ref{tab:pragma} for description of the optimization options.
  }}
    \label{tab:app_details}
  \resizebox{1\linewidth}{!}{%
\begin{tabular}{l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l}
\hline
  \textbf{Application}                  & \textbf{Domain} & \textbf{Major Kernels}     & \textbf{Dataset}    & \textbf{Optimization Space}                                                                     \\ \hline
    blstm~\cite{diamantopoulos2018ectalk} &  \begin{tabular}[c]{@{}l@{}} Machine \\learning\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Hidden layer fw\\ Hidden layer back \\ Output layer\end{tabular} & Fraktur OCR~\cite{yousefi2015binarization} & 
    \begin{tabular}[c]{@{}l@{}}2$\times$PL, 3$\times$PR(2,4), IL, 2$\times$UR \\ 2$\times$PL, IL, 2$\times$UR  \\ PL, IL, UR, DF, BR, BW, FR\end{tabular}

\\\hline 
    
     cedd~\cite{gomezluna2017chai}             & \begin{tabular}[c]{@{}l@{}}  Image \\  proc. \end{tabular}   & \begin{tabular}[c]{@{}l@{}}
     Gaussian filter\\
     Sobel filter\\
    Suppression filter\\
    Hysteresis filter\\
    \end{tabular}            & \begin{tabular}[c]{@{}l@{}}   Frame-354$\times$626 \\ 1000 frames               \\
    \end{tabular}  &
    \begin{tabular}[c]{@{}l@{}}  
    PL, PR(2,4), IL, UR\\
    PL, PR(2,4), IL, UR\\
    PL, PR(2,4), IL, UR\\
    PL, IL, UR, DF, BR, BW, FR\\
    
    
     \end{tabular} 
    \\
\hline 
    digit~\cite{zhou2018rosetta}             & \begin{tabular}[c]{@{}l@{}}  Machine \\learning \end{tabular}    & \begin{tabular}[c]{@{}l@{}}Hamming dist.\\
    KNN voting\end{tabular}          & \begin{tabular}[c]{@{}l@{}} MNIST-18000 train \\
    2000 test  \end{tabular}        &       \begin{tabular}[c]{@{}l@{}}       
     2$\times$PL, 3$\times$PR(2,4), IL, 4$\times$UR\\
IL, BR, BW, FR\\

\end{tabular}
\\\hline 
    
 
    hist~\cite{gomezluna2017chai}                      &\begin{tabular}[c]{@{}l@{}}   Image\\ proc.  \end{tabular}   & Histogram avg.     &    \begin{tabular}[c]{@{}l@{}}   Input-1536$\times$1024      \\
    Bins-256\\
        \end{tabular} & \begin{tabular}[c]{@{}l@{}} PL, PR, IL, DF,\\ BR, BW, UR, FR  \end{tabular} \\
\hline 

     sc~\cite{gomezluna2017chai}                & \begin{tabular}[c]{@{}l@{}}   Data\\ reorg.  \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Count\\ Compact\end{tabular}       &                  1048576 elements    & \begin{tabular}[c]{@{}l@{}}PL, IL, DF, BR, BW, UR, FR       \end{tabular}          \\ \hline
   select~\cite{gomezluna2015ds}         & Database          & Selection                                                                         &     1048576 elements        & \begin{tabular}[c]{@{}l@{}}  PL, IL, DF, BR, BW, FR       \end{tabular}     
   \\\hline 
   
   
% \vspace{-1cm}
\end{tabular}
}
\end{table}


==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/compare.tex <==
 \vspace{0.2cm}
\begin{table}[h]
\centering
  \caption{Average accuracy (\%) comparison of \namePaper~ with decision tree (DT) and adaBoost (ADA) as TL for~\textit{5-shot}~transfer.}
    \vspace{-0.1cm}
    \label{tab:compare}
    \resizebox{0.6\linewidth}{!}{%
\begin{tabular}{@{}llll@{}}
\hline
\textbf{Environment}               & \textbf{DT}   & \textbf{ADA}   & \textbf{\namePaper} \\ \hline
Across Platform       & 77.7 & 83.2 & 89.8  \\
Across Application & 70.6 & 73.5 & 81.2   \\ \hline
\end{tabular}
}
%   \vspace{-0.5cm}
\end{table}

==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/hardware.tex <==
% Please add the following required packages to your document preamble:
% 

\begin{table}[h]
\centering
  \caption{System parameters and configuration.}
    \label{tab:systemparameters}
    \renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{1pt}
    \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lllllr@{}}
\toprule
\multicolumn{5}{l}{\textbf{Low-end Edge System}} & \textbf{Indicative Price}                                                                                                                                                                               \\ \midrule

    & 
\multicolumn{4}{l}{PYNQ-Z1 ZYNQ~\cite{pynq} XC7Z020-1CLG400C~\cite{zynq} with} & \$299\footnote{https://store.digilentinc.com/pynq-z1-python-productivity-for-zynq-7000-arm-fpga-soc/, Accessed 12 Jan. 2021} \\

&\multicolumn{4}{l}{PCIe Gen2~\cite{pcie} ARM Cortex-A9  @650MHz, dual-core} \\ 
&\multicolumn{4}{l}{512MB DDR3 with 16-bit bus @ 1050Mbps} \\ 


\toprule
\toprule
\multicolumn{5}{l}{\textbf{Nimbix Cloud~\cite{nimbix} System with OpenStack\cite{openstack} and KVM Hypervisor~\cite{kvm}}}     & \textbf{Indicative Price}                             \\ \midrule
\textbf{Host Configuration}    & 
\multicolumn{4}{l}{IBM\textsuperscript{\textregistered} POWER9 AC922~\cite{POWER9} @2.3 GHz, 16 cores} & \$55000-\$75000\footnote{https://www.microway.com/product/ibm-power-systems-ac922/} \\ 
&\multicolumn{4}{l}{4-way SMT~\cite{smt}, 32 KiB L1 cache,256 KiB L2 cache,} \\ 
&\multicolumn{4}{l}{10 MiB L3 cache, 32GiB RDIMM DDR4 2666 MHz~\cite{rdimm}} \\ 

\midrule
\textbf{FPGA Description} & \multicolumn{4}{l}{}      &                             \\ 
% \textbf{FPGA Family}      & Zynq            & Virtex UltraScale\tnote{+}            & Virtex UltraScale\tnote{+}            & Kintex UltraScale\tnote{+}            & Kintex UltraScale            & Kintex UltraScale           \\
% \textbf{Board}            &                 & Semptian NSA241                   & ADM-PCIE-9V3                 & N250SP                            & ADM-PCIE-8K5                 & ADM-PCIE-KU3                \\
% \textbf{Device}           &  Z7020-2               & XCVU9P-2                          & XCVU3P-2                     & KU15P-2                           & XCKU115-2                    & XCKU060-2                   \\
% \textbf{Interface}        &                 & CAPI-2                            & CAPI-2                       & CAPI-2                            & CAPI-1                       & CAPI-1                      \\ \bottomrule

 \textbf{Board} &\textbf{FPGA Family}        &\textbf{Device}   &\textbf{Interface}& & \textbf{Indicative Price}      \\    
ADM9V3~\cite{ad9v3}   &Virtex UltraScale\tnote{+} & XCVU3P-2  & { CAPI-2 }   & & N/A  \\
NSA241~\cite{nsa241}& Virtex UltraScale\tnote{+} &XCVU9P-2  & { CAPI-2 }  & & N/A  \\
N250SP~\cite{250SP}&Kintex UltraScale\tnote{+} &KU15P-2  &{ CAPI-2 }  & & N/A  \\     
ADMKU3~\cite{adku3}    &Kintex UltraScale &XCKU060-2  & { CAPI-1 }  & & N/A \\
ADM8K5~\cite{ad8k5}   &Kintex UltraScale &XCKU115-2   & { CAPI-1 }  & & N/A \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\begin{flushleft}
\scriptsize \textsuperscript{5} https://store.digilentinc.com/pynq-z1-python-productivity-for-zynq-7000-arm-fpga-soc/ \ommm{(accessed on 2022-06-13)}\\
\scriptsize \textsuperscript{6} https://www.microway.com/product/ibm-power-systems-ac922/ \ommm{(accessed on 2022-06-13)}\\
N/A: Not available indicative price from an online store, but in the region of \$2500-\$5000 for our purchased on-prem cards.
\end{flushleft}
\end{table}
\vspace{-0.4cm}


==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/jsd.tex <==
 \vspace{0.2cm}
\begin{table}[h]
\centering
  \caption{Jensen-Shannon Divergence (JSD)~\cite{jsd} between %different application's 
  performance distributions of different applications. JSD measures statistical distance between two probability distributions.}
  \vspace{-0.1cm}
    \label{tab:jsd}
     \renewcommand{\arraystretch}{0.9}
% \setlength{\tabcolsep}{1pt}
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{@{}clllllll@{}}
\hline   
\multirow{10}{*}{\rotatebox{90}{\textbf{Target Model}}} & \multicolumn{7}{c}{\textbf{Base Learner}}\\

                              & \multicolumn{1}{l}{}       & blstm & cedd & digit & hist & sc   & select \\ %\cmidrule(l){2-8} 
                              \cmidrule{2-8} 
                              & \multicolumn{1}{l|}{blstm}  & 0.00     & 0.24 & 0.34  & 0.25 & 0.31 & 0.30   \\
                              & \multicolumn{1}{l|}{cedd}   & 0.24  & 0.00     & 0.49  & 0.54 & 0.41 & 0.40   \\
                              & \multicolumn{1}{l|}{digit}  & 0.34  & 0.49 & 0.00      & 0.25 & 0.21 & 0.21   \\
                              & \multicolumn{1}{l|}{hist}   & 0.25  & 0.54 & 0.25  & 0.00     & 0.25 & 0.24   \\
                              & \multicolumn{1}{l|}{sc}     & 0.30  & 0.40 & 0.21  & 0.24 & 0.00     & 0.05   \\
                              & \multicolumn{1}{l|}{select} & 0.30  & 0.41 & 0.21  & 0.25 & 0.05 & 0.00       \\ \hline
\end{tabular}
}
%   \vspace{-0.4cm}
\end{table}

==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

%\vspace{-0.1cm}

\begin{table}[h]
\centering
\caption{Main application features extracted from LLVM.}
\label{tab:application_features}
\centering
\small
 \renewcommand{\arraystretch}{1}
\renewcommand{\baselinestretch}{0.01}
\setlength{\tabcolsep}{10pt}
  \resizebox{1\linewidth}{!}{%
\begin{tabular}{p{0.32\linewidth} p{0.68\linewidth}}
\hline
\textbf{Application Feature} & \textbf{Description} \\ 
\hline
Instruction Mix & Fraction of \ommm{each} instruction type (integer, floating point, memory read, memory write, etc.) \\
ILP                      & Instruction-level parallelism on an ideal machine. \\
Data/Instruction Reuse Distance   & For a given distance $\delta$, probability of reusing one data element/instruction (in a certain memory location) before accessing $\delta$ other unique data elements/instructions (in different memory locations). \\
Register Traffic    & Average number of registers {per} instruction. \\
Memory Footprint    & Total memory size used by the application. \\ 
\hline

\end{tabular}
}
\end{table}


%For a given data distance $\sigma$, the probability that a memory \juan{location} is reused before accessing other $\sigma$ unique memory \juan{locations.} \\
%For a given instruction distance $\delta$, the probability that a memory \juan{location} is reused before accessing other $\delta$ unique memory \juan{locations.}    \\
%The percentage of operations that need to access the next level of memory hierarchy\\
%The average number of register read and write operations \\


==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/pragma_configuration.tex <==
\begin{table}[h]
\centering
  \caption{\gaganT{Accelerator optimization options used in training.}}
%   \caption{ Overview of terms related to the considered FPGA configuration options}
    \label{tab:pragma}
        \resizebox{0.85\linewidth}{!}{%
\begin{tabular}{@{}lll@{}}
\hline
Optimization &  Description  \\ \hline
Loop pipelining (PL)       &   Enabled/disabled \\
Loop unrolling  (UR)     &   Unrolling factor (Factor: $2^n, 1\leq n \leq 6$) \\
Array partitioning (PR)   &  Block/cyclic/complete (Factor: $2^n, 1\leq n \leq 6$)) \\

Inlining (IL)        &   Enabled/disabled function inlining \\
Dataflow (DF)        &  Task level pipelining \\
Burst read (BR)     &   Read data burst from the host \\
Burst write (BW)    &   Write data burst \ommm{to} the host \\

% Replication     &  Kernel duplication factor   \\
FPGA frequency (FR)     &  Four-different frequency levels for an FPGA logic\\ & (50 MHz, 100 MHz, 150 MHz, and 200 MHz)   \\
\hline
\end{tabular}
}
% \vspace{-0.5cm}
\end{table}

==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/timing.tex <==
\vspace{0.3cm}
\begin{table}[h]
\caption{DoE time for gathering sampled data points for a single CPU-FPGA platform (``DoE run (hours)''), DoE execution time on the deployed platform (``Exec (ms)''), Estimated Cost on a cloud platform (``Est. Cost (\$)''), time for gathering 5 labeled samples (``5-shot (hours)''), \namePaper~time including the transfer time (``Transfer (msec)''), ``Speedup'' over building a new model from scratch using only the DoE data%(still {more} cost-efficient than traditional ``brute-force'' training)
.}
\label{tab:timing}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\vspace{-0.1cm}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{p{0.1\linewidth}|lll|lll|l}
% \begin{tabular}{p{0.1\linewidth}|p{0.14\linewidth}p{0.12\linewidth}p{0.14\linewidth}p{0.11\linewidth}}
%\begin{tabular}{p{1.2cm}|p{1.1cm}p{1.6cm}p{1.8cm}p{1.2cm}}
\hline
\multicolumn{1}{c|}{\textbf{Application}}  & \multicolumn{3}{c}{\textbf{Traditional}} &
\multicolumn{3}{c}{\textbf{\namePaper}} &
\\ 

Name &
 \begin{tabular}[c]{@{}l@{}}       
 DoE run \\(hours)

\end{tabular}&
 \begin{tabular}[c]{@{}l@{}}       
Exec \\(msec)

\end{tabular}&
 \begin{tabular}[c]{@{}l@{}}       
Est.Cost$^{7}$\\(\$)

\end{tabular}&
 \begin{tabular}[c]{@{}l@{}}       
5-shot \\(hours)

\end{tabular}
& \begin{tabular}[c]{@{}l@{}}       
Transfer \\(msec)

\end{tabular}&
 \begin{tabular}[c]{@{}l@{}}       
Est.Cost$^{7}$\\(\$)

\end{tabular}
&Speedup\\ \hline




blstm   &  135  &  455 & 168.7 & 13 & 55.6 & 16.2 & 10.4  \\

cedd    &  124  & 295 & 155.0 & 12 & 26.5 & 15.0 & 10.3 \\

digit   & 122   & 435 & 152.5 & 12 & 58.8 & 14.9 & 10.2\\

hist    & 97  &  45  &  121.2 & 9 & 17.1   & 11.3 & 10.8   \\

sc      & 104  & 145 &  130.0 & 10 & 27.9 & 12.4 & 10.4 \\

select  &  106   & 145 & 132.5 & 10 & 27.6 &  12.5 & 10.6
\\

% \bottomrule
   \hline 
   \multicolumn{8}{l}{$^{7}$\small{The cost is estimated based on an enterprise online cost estimator~\cite{nimbix-calc}. Specifically, we selected an}} \\
   \multicolumn{8}{l}{\small{\textit{n2}~(8-core, 64GB RAM VM - 1.25\$/h) for bitstream generation (x86) and an \textit{np8f1} instance (160-thread}} \\
   \multicolumn{8}{l}{\small{1TB RAM, ADM-PCIE-KU3 with CAPI-1 - 3\$/h) for deployment.}} \\
\end{tabular}
}
% \vspace{-0.2cm}
\end{table}

% blstm   &  135  &  9.1 & 13 & 10.1 & 10.4  \\

% cedd    &  124  & 2.9 & 12 & 12.0 & 10.3 \\

% digit   & 122   & 8.7 & 12& 15.3 & 10.2\\

% hist    & 97  &  0.9  &   9& 12.5   &  10.8   \\

% sc      & 104  &   2.9  &  10& 12.7 & 10.4 \\

%select    & 104  &   2.9  &  10& 12.7 & 10.4 \\

==> LEAPER_ICCD'22_Camera_ready_FINAL/tables/values.tex <==
\begin{table}[h]
  \caption{{Execution time and resource \ommm{usage} for low-end edge configuration (PYNQ-Z1) and high-end cloud configuration (Nimbix \textit{np8f1} instance).}}
  \vspace{-0.4cm}
 \label{tab:low_high_end}
% \setlength{\tabcolsep}{2pt}
 \begin{center}
\renewcommand{\arraystretch}{0.85}
%  \renewcommand{\arraystretch}{0.9}
% \setlength{\tabcolsep}{1pt}
  \resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l}
\hline
\textbf{Application} & \textbf{Config.} & \textbf{Exec (msec)} & \textbf{BRAM} & \textbf{DSP} & \textbf{FF} & \textbf{LUT} \\ \hline
\multirow{ 2}{*}{blstm}         &      low-end              &   4200              &    80\%       &    15\%          &     24\%           &   47\%           \\
                                &\ommm{\namePaper}  &   1245              &    62\%       &    8\%          &     12\%           &   21\%           \\

\multirow{ 2}{*}{cedd}          &    low-end                &    10254              &     83\%          &    37\%          &   95\%          &     97\%         \\
                                &   \ommm{\namePaper} &    2217             &   56\%                &      3\%          &   75\%            &              94\%         \\

\multirow{ 2}{*}{digit}         &    low-end                &   2458             &     94\%              &       33\%         &     79\%          &            85\%     \\
                                & \ommm{\namePaper}  &       873          &     84\%              &       12\%         &     24\%          &            75\%              \\

\multirow{ 2}{*}{hist}          &    low-end                &    6173              &      94\%         &     0\%         &     11\%       &         37\%     \\
                                &  \ommm{\namePaper}  &   1104              &     67\%             &    0\%           &    5\%          &             30\%           \\

\multirow{ 2}{*}{sc}            &   low-end                 &   19306              &    82\%       &    0.4\%          &     12\%           &   25\%           \\
                                &\ommm{\namePaper}  &   4018              &    91\%       &    0.1\%          &     12\%           &   23\%     \\
 
\multirow{ 2}{*}{select}        &       low-end              &   18306              &    82\%       &    0.4\%          &     12\%           &   25\%           \\
                                &\ommm{\namePaper}  &   3918              &    91\%       &    0.1\%          &     12\%           &   23\%     \\   \hline
\end{tabular}
}
 \end{center}
\end{table}

==> abstract_submit.tex <==
Machine learning has recently gained traction as a way to overcome the slow accelerator generation and implementation process on an FPGA. It can be used to build performance and resource usage models that enable fast early-stage design space exploration. First, training requires large amounts of data (features extracted from design synthesis and implementation tools), which is cost-inefficient because of the time-consuming accelerator design and implementation process.  Second, a model trained for a specific environment cannot predict performance or resource usage for a new, unknown environment. In a cloud system, renting a platform for data collection to build an ML model can significantly increase the total-cost-ownership (TCO) of a system. Third, ML-based models trained using a limited number of samples are prone to overfitting. To overcome these limitations, we propose LEAPER, a transfer learning-based approach for prediction of performance and resource usage in FPGA-based systems. The key idea of LEAPER is to transfer an ML-based performance and resource usage model trained for a low-end edge environment to a new, high-end cloud environment to provide fast and accurate predictions for accelerator implementation. Experimental results show that LEAPER (1) provides, on average across six workloads and five FPGAs, 85% accuracy when we use our transferred model for prediction in a cloud environment with 5-shot learning and (2) reduces design-space exploration time for accelerator implementation on an FPGA by 10x, from days to only a few hours.

==> images/LHS.tex <==
\begin{SCfigure}[][h]
\vspace{0.8cm}
\centering
    \resizebox{0.3\textwidth}{!}{
    
    
    \begin{tikzpicture}
    %[rotate=90,transform shape]

\draw[step=0.25cm,gray,very thin] (0,0) grid (2,2);

\draw[thick,->] (0,0) -- (2.4,0);
\draw[thick,->] (0,0) -- (0,2.2);
%  \node at (0,0) [circle,fill=black] {};
%  \filldraw [gray] (0,0.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (2,2) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.25,1.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.75,0) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1,1.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.75,0.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.5,0.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.25,1.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0,1) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.5,0.5) circle (2pt);


 
 
\node at (0,2.4)[ rotate=0] {\small \textit{x1}};
\node at (2.6,0)[ rotate=0] {\small \textit{x2}};
\end{tikzpicture}
}
\vspace{-1cm}
\caption{LHS with 2 parameters where the input space is divided into equal intervals and 9 non-overlapping sample points are chosen.
\label{fig:LEAPER_SIGMETRICS/LHS}}
\end{SCfigure}

